Feasibility of a directional solar neutrino measurement with the CYGNO/INITIUM experiment

Over the past five decades, solar neutrino research has been pivotal in driving significant scientific advancements, enriching our comprehension of both neutrino characteristics and solar processes. Despite numerous experiments dedicated to solar neutrino detection, a segment of the lower pp spectrum remains unexplored, while the precision of measurements from the CNO cycle remains insufficient to resolve the solar abundance problem determined by the discrepancy between the data gathered from helioseismology and the forecasts generated by stellar interior models for the Sun. The CYGNO/INITIUM experiment aims to deploy a large 30 m3 directional detector for rare event searches focusing on Dark Matter. Recently, in the CYGNUS collaboration, there has been consideration for employing these time projection chamber technology in solar neutrino directional detection trough neutrino-electron elastic scattering. This is due to their potential to conduct low-threshold, high-precision measurements with spectroscopic neutrino energy reconstruction on an event-by-event basis driven by the kinematic. However, so far, no experiments have been investigated on the feasibility of this measurement using actual detector performances and background levels. Such a detector already with a volume of O(10) m3 could perform an observation of solar neutrino from the pp chain with an unprecedented low threshold, while with larger volumes it could measure the CNO cycle eventually solving the solar metallicity problem.

==> chapters/CYGNO.tex <==
%----------------------------------------------------------------------------------------
%	Research Proposal
%----------------------------------------------------------------------------------------
\chapter{The CYGNO/INITIUM experiment}
\label{chap:CYGNO}
The CYGNO experiment is developing an innovative approach for directional dark matter (DM) and rare events involving low-energy interactions. CYGNO employs a high-resolution Time Projection chamber, operating with a helium-tetrafluoromethane gas mixture at atmospheric pressure and room temperature. The setup uses Gas Electron Multipliers (GEMs) operated with optical sensors for amplification and readout. In particular, to image a large detection area with high granularity using a reduced number of readout channels Scientific CMOS (sCMOS) cameras are used. the peculiar goal of the ERC Consolidator Grant INITIUM is to develop negative ion drift operation (see Sec. \ref{sec:NID}) at atmospheric pressure within the CYGNO experimental approach. The two projects' results therefore extremely synergic and the development and characterisation of their prototypes and detectors proceeded together.\\ 
The combination of sCMOS camera images with the signals provided by photomultiplier tubes (PMTs) allows for particle 3D reconstruction with directional capabilities and sense recognition, at energies down to $\mathcal{O}(1)$ keV. A complete overview of the CYGNO experiment can be found in \cite{instruments6010006}. Since the beginning of the project, many prototypes have been developed with a scaling up in dimensions. This approach aims to solidify the experimental technique, refine the performances, and study the scalability of the optical gas TPC approach. The objective of CYGNO is to construct a detector with a volume of $\mathcal{O}(10-100)\ m^3$ in underground facilities, to be competitive in dark matter searches and solar neutrino spectroscopy with the unique feature of the directional sensitivity. Additionally, CYGNO is part of the CYGNUS project, which aims to establish a multi-site Galactic Recoil Observatory, that can probe dark matter hypotheses beyond the "neutrino fog" (once "neutrino floor") \cite{O_Hare_2021}, and measure neutrinos from the Sun and supernovae with a directional approach. At the moment the CYGNO collaboration comprises approximately 50 researchers from institutions across four different countries: Italy, Portugal, Great Britain, and Brazil. 
In this Chapter, a comprehensive description of the CYGNO technique is provided (Sec. \ref{sec:CYGNOTec}). This will be followed by 
a description of multiple physics cases to which the innovative technique of CYGNO can be applied (Sec. \ref{sec:PhysCase}). Subsequently, a timeline overview (Sec. \ref{sec:Timeline}) with a particular focus on the latest prototype LIME (Sec. \ref{sec:LIME}) and the latest results will be given. Afterward, an illustration of the MANGO prototype, employed to carry on parallel research lines for the experiment (Sec. \ref{sec:MANGO}) will follow, to finally expose the future project and plans of the CYGNO experiment (Sec. \ref{sec:CYGNOFut}). 

\section{The CYGNO tecnique}
\label{sec:CYGNOTec}
The aim of the CYGNO collaboration is to deploy a high-resolution detector for directional DM searches and rare events. The detector relies on a gaseous Time Projection Chamber (TPC) using a scintillating helium and fluorine based gas mixture, operated at room temperature and atmospheric pressure. The amplification stage consists of three 50 $\mu m$ Gas Electron Multipliers (GEMs) and is optically readout using scientific Complementary Metal-Oxide-Semiconductor (sCMOS) cameras and Photomultiplier Tubes (PMTs). 
TPCs are detectors consisting of a sensitive volume enclosed between two electrodes: a cathode and an anode, these elements generates electric field inside the sensitive volume, that is maintained homogeneous by a field cage \cite{10.1063/1.2994775, Nygren:1974nfi, ATWOOD1991446}. Typically, the anode of the TPC is instrumented with a readout system, but also the cathode can be instrumented. In figure \ref{fig:tpcscheme} a schematic view of a TPC is shown, with its key components. 
\begin{figure}
    \centering  \includegraphics[scale=.5]{figures/TPCScheme.png}
    \caption{Illustration of a Time projection chamber highlighting its key features. Given its 3D nature, it allows for particle identification and head-tail recognition, exploiting the track topology. }
    \label{fig:tpcscheme}
\end{figure}
The passage of an ionizing particle inside the sensitive volume creates a trail of electrons-ions pair along its trajectory. The electric field in the active gas volume prevents electrons from recombination with ions, causing them to drift toward the anode. Given that the charge generated during ionization is often too small for direct detection, a stage of amplification is commonly placed at the anode to amplify the primary electron charge. The amplified signal can be recorded using various technologies, and their interplay with gas properties, such as density and scintillation properties, significantly impact the detector performance. TPCs are by construction 3D detectors, with low energy threshold, due to the small ionizing power needed to create an electron-ion pair ($\mathcal{O}(10s eV)$), and thus suitable for low energy electron and nuclear recoil tracking. The detector concept of CYGNO integrates 4 pioneering elements explained in the following points:
\begin{itemize}
    \item The target gas is made up of a mixture of He and CF$_4$. This multi-target gas mixture enables concurrent sensitivity to both SI and SD coupling to DM. Additionally, CF$_4$ has scintillation properties which are optimal for an optical readout. The chosen 60:40 proportion ensures a low gas density, roughly comparable to that of air, and ensures stability in long term detector operations. This allows electron and nuclear recoils to travel longer distances, facilitating the directional reconstruction.
    \item The amplification stage consists of three 50 $\mu m$ thick Gas Electron Multipliers (GEMs). These objects are a type of micro-pattern gas detectors (MPGDs), which provide significant charge amplification gain, enabling low energy thresholds, and offer high granularity, aligning well with the sCMOS camera sensor and optical system used in the CYGNO setup \cite{knoll2010radiation, SAULI20162}. Moreover, GEMs are one of the few MPGDs that can be manufactured in large dimensions, a crucial requirement for the upcoming stages of the experiment (Sec. \ref{sec:CYGNOFut}).
    \item The amplified signal is optically read out using both PMTs and sCMOS cameras. Optical sensors, in general, offer a significantly higher signal-to-noise ratio compared to charge detectors, enhancing detection efficiency. sCMOS cameras provide a highly granular 2D readout at a reasonable cost, with a high quantum efficiency in the optical band, making them suitable for imaging large areas when coupled with appropriate lenses (Sec. \ref{sec:camera}). %Additionally, the camera readout takes place with a simple USB 3.1 cable, and this facilitates a lot the channel management. 
    With their longer acquisition times, sCMOS cameras effectively yield a 2D projection of all the recoil tracks, on the GEM plane, allowing for the extraction of tracks topology and directional information. %Additionally, the camera offers a measurement of the deposited energy, which is proportional to the photons collected by the sensor. 
    The PMTs sample the light produced by the track while primary electrons gradually arrive at the amplification plane. The PMT (Sec. \ref{sec:PMT}), thus, is able to keep track of the z coordinate of the track.
    Combining the sCMOS camera with PMTs enables the accurate measure of the track energy using two distinct photosensors. %Furthermore, by integrating the 2D information provided by the sCMOS camera with the data in the orthogonal directional obtained from the PMTs a full 3D reconstruction of the track can be reached. The ability to reconstruct the 3D topology of recoils is particularly valuable, allowing for effective discrimination between ER and NR, and for 3D direction measurement of the track. 
    While the solid angle coverage, affecting the number of photons reaching the optical sensors, is limited, this is effectively balanced by the considerable gain achievable through the GEM amplification structure (Sec. \ref{sec:GEM}).
    \item The ability to operate at atmospheric pressure. It ensures a favorable volume-to-target-mass ratio, simultaneously reducing engineering demands on the realization of a gas-tight vessel and minimizing internal backgrounds. Among all the directional detectors, CYGNO stands out as the only detector, apart from $D^3$ \cite{Ahn_2022} where the prototypes never exceed 0.3 liters in active volume, to operate at atmospheric pressure. This enhances the experiment's exposure without compromising the recoil track lengths, given the low gas density.
\end{itemize}


\subsection{Choise of the gas mixture}
\label{sec:gasmixture}
The gas mixture selection takes a central role as it strongly influences the experimental properties of the detector and delineates the target for the physics searches. Tetrafluoromethane, CF$_4$, is a scintillating gas known for its high light yield within the visible spectrum, even when combined with noble elements \cite{LMMargato_2013,FRAGA200388,AMorozov_2012,KMPZMT_CF4Trasnp}. The emitted light spectrum exhibits two distinct continua, the first peaking around 290 nm (UV region) and the second at 620 nm (visible region). Emission within the visible orange region stems from the de-excitation process of a Rydberg state of the neutral CF$_3^{*-}$, resulting from CF$_4$ fragmentation, with an associated energy threshold of 12.5 eV. Conversely, the dissociative ionization threshold is 15.9 eV, and numerous resulting ionic fragments from CF$_4$ fragmentation emit within the UV band. Gas mixtures incorporating CF$_4$ display remarkably low diffusion during the drift phase \cite{SAULI20162}, attributable to the substantial characteristic scattering cross-sections of electrons with CF$_4$.\\
A low diffusion coefficient of the electrons in the gas is a factor that permits to maintain high-quality 3D tracking of a Time Projection Chamber (TPC). Having a lower diffusion allows the realization of a detector with a longer drift field (thus a larger volume) while maintaining the same tracking performance. In the CYGNO experiment, Helium (He) is combined with CF$_4$ in the gas mixture. Helium, being a noble gas, is chemically stable and inert, making it practical for use in particle detectors. Additionally, when combined with other molecular gases, helium can provide large amplification, as evidenced in prior studies \cite{SAULI20162}. The strategic combination of the very low density of Helium with CF4 scintillation properties allows CYGNO to operate at atmospheric pressure while maintaining an overall target density only approximately twice as large as that of the NEWAGE experiment, which operates with pure CF$_4$ at 100 Torr of pressure \cite{10.1093/ptep/ptab053}. \\
%In the physics of direct dark matter detection, the reduced mass WIMP-target system and the experimental energy threshold play a crucial role in defining the minimum DM mass to which an experiment is sensitive. Opting for a light target with atomic mass A < 10, coupled with a typical $\mathcal{O}$(1) keV energy threshold can potentially extend the experiment sensitivity to DM masses below 10 GeV, a portion of the parameter space that remains largely unexplored to date. For reduced mass reasons, the He used in the CYGNO gas mixture with $A=4$, lead to the maximization of the sensitivity to WIMP masses of a few GeV for SI couplings. Additionally, the favorable kinematic compatibility of He with WIMP of low mass, coupled with its light mass, results in longer NR produced after an interaction compared to heavier target elements, leading to better performances in the measurement of track directionality and head-tail recognition. Moreover, the abundant presence of fluorine atoms in CF$_4$ enables sensitivity to SD couplings, particularly at low WIMP masses close to the Fluorine mass. Consequently, thanks to its gas chemical composition, CYGNO stands out as one of the rare experiments in the DM detection field able at the same time to search both SI and SD interactions at low WIMP masses.\\
A study of optimization was carried out to determine the optimal He:CF4 ratio that would enhance the gain and light production in the experimental approach of CYGNO, while simultaneously minimizing diffusion and detector instabilities. A ratio of 60:40 was identified as the most suitable as reported in \cite{Baracchini_2020_Stab,Campagnola:2313231}. The transversal and longitudinal diffusion coefficient per unit of length traveled by the electrons, and the drift velocity as a function of the electric field, calculated using the Garfield software of simulation \cite{Veenhof:1993hz,VEENHOF1998726} are reported in figure \ref{fig:diffvel}.
\begin{figure}
    \centering
    \includegraphics[scale=.40]{figures/DiffVsE.png}
    \caption{Left/Center: Transversal/Longitudinal diffusion for electrons in a He:CF$_4$ mixture 60:40 and 70:30 simulated with Garfield++. Right: plot of the electron drift velocity as a function of the drift field intensity from Garfield++ simulation.}
    \label{fig:diffvel}
\end{figure}
From the simulation \cite{Baracchini_2020_Stab}, it is obtained a diffusion coefficient for both longitudinal and transversal diffusion below 140 $\mu$m/$\sqrt{cm}$ in a range of electric field of $[0.5, 1]\ kV/cm$. This can be compared with the diffusion of Ar:CF$_4$ of around 600 $\mu m/\sqrt{cm}$\cite{ParticleDataGroup:2020ssz}. The drift velocity is estimated to be $\sim \ 3-6 cm/\mu s$ in the same range. The energy required in the gas mixture to produce a single electron-ion pair (namely the w-value) results in average $\sim 38 \ eV$ \cite{Workman:2022ynf}. To further reduce diffusion, Negative Ion Drift (NID) studies are in progress in the context of the INITIUM project. The characteristics of this peculiar modification in the TPC operation are described in Sec. \ref{sec:NID}, including the first successful demonstration of its feasibility at atmospheric pressure within the CYGNO readout strategy. \\
Finally, the electron and He ion recoil ranges have been simulated using the GEANT4 toolkit \cite{AGOSTINELLI2003250} and the SRIM software \cite{Ziegler1985}, respectively in the CYGNO gas mixture.
The mean 3D ranges, namely the distance in a straight line between production and absorption points, as a function of the kinetic energy of He nuclei and electrons are shown in Figure \ref{fig:ranges}. It can be observed from the picture that the range of Helium recoils is below a few millimeters up to 100 $keV_{nr}$, resulting in the creation of a dense and bright spot slightly asymmetric in the recoil direction that preserves the directional information. Contrarily electrons can travel many $cm$ inside the gas volume before getting absorbed.
\begin{figure}
    \centering
    \includegraphics[scale=.3]{figures/ERNRRange.png}
    \caption{Average 3D range for He recoils and electrons recoils as a function of their kinetic energy.}
    \label{fig:ranges}
\end{figure}

\subsection{Triple gem amplification system}
\label{sec:GEM}
%The amplification stage of CYGNO consists of a stack of GEMs. The use of an optical readout reduces the signal intensity due to limited solid angle coverage (Sec. \ref{sec:optics}). As a consequence of this, a significant amplification of the number of primary charges is necessary to achieve suitable gain for detecting low-energy events.
Among the gas detectors capable of providing high gains, GEMs are highly performing. GEMs represent a specific implementation of Micro Pattern Gas Detectors (MPGD), initially designed to enhance spatial granularity and efficiency with respect to wire chamber detectors, especially in the presence of high particle fluxes \cite{knoll2010radiation,SAULI20162}. This device was projected by Sauli in 1997, a detailed examination about their characteristics and features can be found in \cite{SAULI20162}. A GEM is composed of a thin, strongly insulating polymer layer coated with conductive metal on the two sides, with a high density of equispaced holes. When a significant potential difference is applied across the two electrodes, high electric fields of approximately $\mathcal{O}$(10) kV/cm are produced within the holes. These fields are strong enough to trigger avalanches when a single electron crosses the holes. The ions generated during the avalanche are primarily captured by the upper metallic surface, mitigating ion back-flow in the drift region and ensuring stable operations, even in high-rate environments \cite{Tripathy:2021puz}. The materials used to fabricate GEMs can vary, but the most commonly used materials include fiberglass or Kapton$^{TM}$ for the insulating layer and copper for the coating. However, ongoing advancements are being made in exploring alternative materials for the insulating layers of GEMs to reduce radioactivity content \cite{pr11041215}.  GEMs can be manufactured with a range of thicknesses, from a very thin 50 $\mu$m up to 1 mm. In the case of thinner GEMs, the hole diameter is typically 70 $\mu$ m wide, as smaller holes do not significantly enhance the effective gain due to an exceedingly high charge density in the hole \cite{SAULI20162}. The pitch between holes is typically around 140 $\mu$m. A hole of this size is realized through a  technique called etching, consisting of precise chemical excavation of tiny holes in materials. The etching procedure applied to GEMs yields to a double-conical geometry for the hole, with the slimmer diameter at its center. In the case of thicker GEMs, both the pitch and hole diameter are proportionally increased. In the case of GEMs thicknesses exceeding 300 $\mu$m, holes can be initially created via mechanical drilling and then further refined using wet etching, which produces finally the double-conical geometry. The precise localization of avalanches within these GEM holes enables exceptional granularity, especially pronounced in the 50 $\mu$m thin ones, largely preserving the x-y topological characteristics of the primary electron cloud. The secondary electrons generated by a GEM during the amplification process can either be collected by an anode or directed to another GEM for additional amplification. Indeed, the use of multiple GEMs stack has been explored and researched for various applications, achieving gains of $\mathcal{O}(10^4-10^6)$ \cite{SAULI20162,GEMOptRead}.\\ The amplification stage of CYGNO consists of a stack of GEMs. The use of an optical readout reduces the signal intensity due to limited solid angle coverage (Sec. \ref{sec:optics}). As a consequence of this, a significant amplification of the number of primary charges is necessary to achieve suitable gain for detecting low-energy events. Ongoing R\&D efforts are focusing on further optimizing and customizing the amplification structure for the CYGNO experiment
are in progress.

\subsection{Optical readout}
\label{sec:optics}
Luminescence in gases is a thoroughly investigated and identified phenomenon. When charged particles move through the gas, they can ionize atoms and molecules and also excite them. As these particles undergo de-excitation, they emit photons. The quantity and spectrum of the produced light are significantly influenced by the gas mixture content, its density, and the presence and intensity of the electric field applied. In typical gas mixtures, the emission can range between $10^{-2}$ and $10^{-1}$ photons per electron in the avalanche \cite{knoll2010radiation,LMMargato_2013,FRAGA200388,MONTEIRO201218}. \\
The optical readout approach consists of detecting the light produced in the amplification processes, a concept pioneered in 90's studies involving parallel plates detector \cite{optReadFirst}. Charge readout poses challenges for detecting extremely low energy deposits since it is often accompanied by electronic noise. The mitigation of this noise requires foresight in the design of the detector and the electric circuits. On the other hand, optical sensors can rely on significantly higher signal-to-noise ratios due to the extremely lower noise level. Additionally, since the optical sensor is decoupled from the rest of the detector it doesn't require particular foresight in the readout configuration. Moreover, employing optical readout enables the placement of the readout sensors outside the sensitive volume, minimizing radioactivity and gas mixture contamination. Nevertheless, this positioning advantage comes with the trade-off of the reduction of the total light acquired, due to limited solid angle coverage. \\ 
As a directional detector, CYGNO's objective is to measure both the direction and energy of recoils. To achieve optimal assessment of the recoil direction and head-tail (HT) orientation, a comprehensive 3D analysis of the track is crucial. This goal is performed through the contemporary employment of two optical sensors: a scientific CMOS (sCMOS) camera that measures the energy release along the x-y projection of the tracks, and a set of PMTs that measure the integrated energy and samples the track development along the drift direction (z-axis).

\subsubsection{The sCMOS camera}
\label{sec:camera}
A scientific CMOS camera (sCMOS) is a highly sensitive, low-noise photon detector belonging to the active pixel sensors (APS) family. It employs the complementary metal-oxide semiconductor (CMOS) pinned photodiode (PPD) technology. CMOS, represents the technology used to fabricate the MOSFET transistors, which are the fundamental building blocks of modern electronics \cite{behzad2001design}.
An active pixel sensor is a silicon-based photodetector that actively handles and readout the charge generated from photon conversion within the depleted region of the sensor. When a photon interacts in the depleted region of the APD an avalanche is created and the current causes a drop of voltage in the sensor. The signal from the APD is typically determined by calculating the difference between the voltage value within the depleted region at the beginning of the integration time and its value at the end.
Within the APS family, a pinned photodiode is a type where the active charge handling is achieved through a combination of n and p-doped silicon architectures. PPDs can be miniaturized to very small dimensions, typically around $\mathcal{O}(10)$ $\mu$m per side. This small size enables the arrangement of PPDs in arrays and matrices, forming highly granular photodetectors or camera sensors. Well-known examples of PPD-based camera sensors include CCD and CMOS cameras \cite{6742594}. \\
In CCD, a semiconductor structure connects each PPD pixel. This structure, at sensor readout time, is used to transfer the charge collected by each pixel to its neighboring pixel using a shift register technique. During each charge transfer step, the information held by the pixels is transferred to the adjacent pixel toward the sensor's boundary. On the sensor border, a circuit is situated to read out the charge transported by each pixel while it progressively arrives. This process of transport continues until all the pixels have been read out \cite{vorobiev2019direct}.\\
Contrarily, CMOS cameras utilize the arrangement where each PPD pixel has its own amplifier and is connected to a specific CMOS circuit designed primarily for direct signal readout. This CMOS circuit is responsible for not only reading the signal but also for pixel reset, noise reduction, and eventual exposure control in certain implementations \cite{6742594}.\\ %The basic configuration involves 4 CMOS transistors, although contemporary CMOS circuitry can incorporate additional CMOS elements to ensure low noise measurements .
CCD cameras typically exhibit superior light collection efficiency and more uniform performance compared to CMOS cameras, because of the depth of the depleted pixel region and the distinct readout approach. Historically, CCDs maintained a lower noise level, but recent advancements in CMOS circuitry have significantly enhanced CMOS capabilities, surpassing CCD performances, particularly in scientific applications (sCMOS). These improvements regard mainly studies of intrapixel effects, and development of dedicated suppression systems, and better modeling of the intrinsic sensor noise for its correction \cite{Zhan_2017,boyat2015review,konnik2014high}.\\
Furthermore, in most applications, CCD sensors necessitate lower operating temperatures than CMOS sensors to mitigate intrinsic noise. In an sCMOS sensor, the individual amplification and readout of each pixel results in thermal noise affecting only that specific pixel. Conversely, in CCDs, the shift register technique leads to the accumulation of thermal noise across multiple stages of the shift. Therefore, CCD sensors generally demand a lower operational temperature compared to sCMOS sensors \cite{2022stiibook21P,Petitdidier813843}. 
CMOS cameras are more cost-effective to manufacture and can have smaller-sized pixels, providing exceptionally high granularity. Additionally, sCMOS cameras maintain lower power consumption than CCDs due to the lower voltages needed to power the sensors compared to the voltages required for the shift register in CCDs. During the readout process indeed, the sCMOS camera is required to provide power to the single-pixel amplifier. This requires a lower voltage compared to the one needed for establishing a voltage difference along the entire pixel lines in the shift register of the CCD. This results in lower power consumption.\\
It's crucial to underline that these types of cameras have a diverse range of applications in the market. For example, CMOS image sensors are used for cellphone cameras because of their reduced noise levels at room temperature and lower power consumption. Therefore, the rapid advancement of sensor technology is driven by market industry demands. Given its advantages of low noise, high granularity, and significant potential for technological advancements, the sCMOS technology has been established for the CYGNO experiment readout.
\\
CYGNO utilizes CMOS cameras manufactured by the Hamamatsu Corporation. Over time, the collaboration tested newer, high-performance models, the main features of which are shown in Table \ref{tab:camersa}. The different acquisition modes are related to the time that the camera employs to expose the sensor to the light. The evolution of technology is evident in the increase in pixel number and reduction in pixel size. Notably, recent models demonstrate a significant reduction in the noise RMS for each pixel, which directly translates into a lower threshold for the detector. Specifically, the noise RMS in the QUEST model is impressively low at 0.27 electrons, enabling the precise counting of photons converted in a pixel shown in figure \ref{fig:ReadNoise}.
\begin{table}[!ht]
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
        Camera Model & Orca Flash & Orca Fusion & Orca Quest \\ \hline
        Pixel number & 2048$\times$2048 & 2304$\times$2304 & 4096$\times$2304 \\ \hline
        Pixel Size ($\mu m^2$) & 6.5$\times$6.5 & 6.5$\times$6.5 & 4.6$\times$4.6 \\ \hline
        RMS Noise (Fast mode) & 1.6 & 1.4 & x \\ \hline
        RMS Noise (Slow mode) & 1.4 & 1.0 & 0.43 \\ \hline
        RMS Noise (Ultra quiet mode) & x & 0.7 & 0.27 \\ \hline
        Max Frame Rate (Fast) & 100 & 89.1 & x \\ \hline
        Max Frame Rate (Slow) & 30 & 23.2 & 120 \\ \hline
        Max Frame Rate (U.Q.) & x & 5.4 & 5 \\ \hline
    \end{tabular}
    \caption{Characteristics of the different cameras tested by the CYGNO collaboration}
    \label{tab:camersa}
\end{table}
The figure shows the simulated p.d.f. of the camera response obtained for a Poissonian distribution of photoelectrons produced per pixel (with an average number of photoelectrons $\lambda=2$) convoluted with the noise of the camera. 
\begin{figure}
    \centering
    \includegraphics[scale=.23]{figures/ReadoutNoise.png}
    \caption{In figure, the probability density function of the number of photoelectrons for different readout noise (different colors) is shown. }
    \label{fig:ReadNoise}
\end{figure}
As can be seen from the picture, the readout noise level of the QUEST (indicated by the red line) is the only one enabling differentiation of signals arising from the different numbers of photons, allowing for direct photon counting. Hence, this new class of sCMOS is often referred to as quantitative CMOS (qCMOS) cameras.\\
As the photon-sensitive region is constructed from silicon, the sensitivity of sCMOS cameras is determined by the bandgap of the silicon crystal, representing the energy difference between the valence and conduction bands. With a minimum bandgap value of 1.12 eV, silicon semiconductors demonstrate limited sensitivity in the infrared region, since the energy is not enough for the transition. Since visible light energy instead, matches the energy range of the bandgap it can promote an electron from the valence band to the conduction one. This characteristic makes silicon an optimal material for detecting visible light. In contrast, as light energy increases into the ultraviolet region, it becomes too high for the transition, causing the excited electron to dissipate its energy within the material. As a result of this sCMOS cameras exhibit high sensitivity within the optical spectrum, while they are insensitive to UV and IR.
The Quantum Efficiency (QE) can peak at around 80\% at approximately 600 nm. This matches well with the emission peak in the visible range for the He:CF$_4$ gas mixture used in CYGNO. In Figure \ref{fig:QE}, the Quantum Efficiency (QE) of the ORCA Fusion is shown, together with the QE of the PMT R7378, a bialkali borosilicate PMT \cite{PMTHamam} used in LIME (Sec. \ref{sec:PMT}). Additionally, the emission spectrum of the CYGNO gas mixture, as measured in \cite{FRAGA200388}, is presented. All the distributions are normalized to 1. It's worth noting that the sCMOS sensor exhibits a significantly higher QE compared to conventional PMTs.
\begin{figure}[h]
    \centering
    \includegraphics[scale=.4]{figures/QeVslambda.png}
    \caption{In figure the quantum efficiency as a function of the wavelength is shown for the Orca Fusion camera (blue) and the PMT R7378 (red) from Hamamatsu. Additionally, the emission spectrum of the He:CF$_4$ 60:40 gas mixture is presented (black).}
    \label{fig:QE}
\end{figure}

\subsubsection{Optical system}
Contemporary sCMOS cameras equipped with megapixel 2D arrays enable the imaging of extended areas when paired with suitable optical systems. Specifically, it is feasible to capture images of areas of $\mathcal{O}$(0.1 $m^2$) using a single camera, all while maintaining excellent granularity of the same order of the segmentation of the GEM amplification stage. The lens employed for all CYGNO detectors is a Schneider Xenon lens with a focal length $f$ of 25.6 mm, an aperture ratio $N$ (f-number) of 0.95, and an optical transparency of 0.85 in the visible range. To capture images of 30$\times$30 $cm^2$ areas using this optical system, the sensor must be placed approximately 20 cm away from the surface of the closest GEM. 
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/LensScheme.png}
    \caption{Diagram illustrating a lens in the Gaussian approximation, adapted from \cite{10.1088/978-0-7503-2558-5}. The yellow cones represent the photons emitted from the object plane (OP) and focused onto the sensor plane (SP).}
    \label{fig:OptSystem}
\end{figure}
Figure \ref{fig:OptSystem}, shows a schematic representation of an optical system with a thick lens in Gaussian approximation projected onto the plane formed by the optical axis (connecting object and sensor and passing through the center of the lens) and the perpendicular axis \cite{10.1088/978-0-7503-2558-5}.
In the picture, OP designates the object plane, housing the focused source, while SP denotes the sensor plane, the location of the photosensor. EP and XP represent the entrance and exit planes, respectively, through which photons enter and exit the lens. H and H' designate the hyperfocal planes, representing the position of a thin lens possessing the optical characteristics of a thick lens. D represents the aperture radius of the lens, determining the surface area designated to receive photons. The infinitesimal element of area emitting photons is denoted as dA, with u representing the tangent of the opening angle. The variables s and s' indicate the distances between the object and the hyperfocal plane H, and between the sensor and the hyperfocal plane H', respectively. Additionally, $f_F$ represents the focal distance, and $F$ represents the focal point. The illustration depicts the operation of a typical thick lens. Photons within the yellow region on the left of EP are captured by the lens and focused onto the sensor. When OP, EP, XP, and SP are parallel, the flux of photons ($\phi$) reaching the lens, emitted from the area $dA$, can be assessed as:
\begin{equation}
    \phi = \pi L u^2 \ dA
    \label{eq:flux}
\end{equation}
where L is the absolute luminosity of the source \cite{10.1088/978-0-7503-2558-5}. The lens's coverage of the solid angle fraction, denoted as $\Omega_f$, can be found by using eq. \ref{eq:flux} and dividing it by the total solid angle of photon emission, which is $4\pi$.
\begin{equation}
    \Omega_f = \frac{\phi}{L\ dA} \frac{1}{4\pi} = \pi u^1 \frac{1}{4\pi} = \frac{(D/2)^2}{4s^2}
    \label{eq:solidang}
\end{equation}
The connection between distances $s$ and $s'$, and the magnification I (process of enlarging the apparent size) can be treated as analogous to the linear optics under the condition $s$ $>>$ $s_{ep}$, where $s_{ep}$ represents the distance between the entrance plane and the hyperfocal plane. In the context of CYGNO optical system, this condition holds, and  it can be affirmed that:
\begin{equation}
    1/f = 1/s +1/s' \ \ \ \ \ \ \ \ I = y'/y = s'/s
    \label{eq:magnific}
\end{equation}
with y and y' the size of the object and the size of the image respectively \cite{1987opt2.bookH}. By combining eq. \ref{eq:solidang} and eq. \ref{eq:magnific} the following expression for the solid angle can be derived:
\begin{equation}
    \Omega_f = \frac{1}{( 4N(\frac{1}{I}+1) )^2}
\end{equation}
where N is the focal number defined as $N=D/f$.
The standard solid angle seen by the Schneider lens and, for instance, the ORCA Fusion camera (as shown in the second row of Table \ref{tab:camersa}) during the imaging of a 30$\times$30 $cm^2$ area is on the order of $10^(-4)$. This factor importantly diminishes the number of photons reaching the sensor. Consequently, a very high gain is necessary from the amplification stage, leading to the use of a stack of three GEMs (Sec. \ref{sec:GEM}).

\subsubsection{The Photomultiplier Tube (PMT)}
\label{sec:PMT}
The Photomultiplier Tube (PMT) is a photon-detecting device with origins dating back to the '30s \cite{PMTHamam}. Its main feature is the single photon sensitivity together with the capability of maintaining a wide dynamic range. The PMT consists of a glass tube under vacuum, comprising an input window covering a photocathode on one extremity and a readout anode on the other extremity. The photocathode is made of a highly photosensitive material, and it is responsible for converting the photons impinging on it into electrons through the photoelectric effect. Within the tube, a series of electron multipliers known as dynodes are present. These dynodes, kept at progressively increasing voltage levels, emit multiple electrons upon being hit by an accelerated electron. Thus, electric fields created between the dynodes accelerate the electrons toward the dynode surface. In each interaction with the dynodes, three to four additional electrons are emitted by the dynode for every incident electron. This avalanche process results in a significant amplification of the signal. At the end of this chain, an anode collects the whole amount of electrons and it is connected to an output cable for signal readout. A scheme of the PMT is shown in figure \ref{fig:PMTScheme}.
\begin{figure}
    \centering
    \includegraphics[scale=1.2]{figures/PMTScheme.png}
    \caption{Working scheme of a PMT with all its key components highlighted.}
    \label{fig:PMTScheme}
\end{figure}
The dynamic range and gain achieved as high as $10^6$ depends on the number of dynodes, their composition, and the voltage divider. The quantum efficiency for different wavelengths (QE) of the PMT is influenced by the materials used for the window and photocathode. Typically, windows are crafted from borosilicate glass, allowing photons above 300 nm to pass through, and can be produced with relatively low radioactive materials. The most common materials used for the production of photocathode are bialkali, typically Sb-K-Cs, named by the presence of more than one alkali element. The QE of these photocathodes reaches its peak at 400 nm, remaining sensitive up to 650 nm. Alternative materials such as GaAsP(Cs) exhibit higher QE within the visible range. In any case, the PMT quantum efficiently does not exceed $\mathcal{O}$(30\%) at the peak.\\
When used in TPCs employing optical readout, analyzing the current signal generated at the anode due to detected photons yields valuable information. The overall charge readout at the anode is directly proportional to the number of photons converted, providing thus a measurement of the energy. The energy resolution, influenced by the QE and photocathode dimensions, can vary, and in cases of low-energy depositions, the main factor affecting energy resolution is typically the variation in the primary electrons generated within the detector's sensitive region.
With a typical PMT single photoelectron time of $\mathcal{O}(ns)$, employing a sampling rate of $\mathcal{O}(GS/s)$ ($10^9$ samples per second) on the PMT waveforms allows for a comprehensive characterization of the waveform. This can allow the study of the track's progression along the drift direction, considering the standard electron drift velocities. This capability can enable not only the determination of the recoil's inclination concerning the GEM plane but can also provide essential insights into the track's topology, crucial for recognizing direction and HT (head-tail) information. Figure \ref{fig:PMTSign} illustrates examples of PMT waveforms for a track that is parallel and tilted concerning the GEM plane, presented in the left and right panels, respectively.
\begin{figure}
    \centering
    \includegraphics[scale=.2]{figures/ParallelPMT.png}
    \includegraphics[scale=.2]{figures/TiltedPMT.png}
    \caption{Left: signal of a track parallel to the GEM plane. Right: signal of a track tilted with respect to the GEM plane. In the first case, the electrons drifting will arrive at the amplification stage in a very short time window releasing all the light in this time window. In the second case they will release the light in a larger time window which depends on the track extension in z.}
    \label{fig:PMTSign}
\end{figure}

\section{CYGNO physics case}
\label{sec:PhysCase}
CYGNO has been mainly developed for directional DM searches, although the experimental approach of optical readout TPC can be applied to many physics cases. These cases include events in which the particle interaction presents a peculiar topological signature in the detector, such as the Migdal effect (Sec. \ref{subsec:migdal}) or the X-ray polarimetry (Sec. \ref{subsec:polarimetry}) case, or events for which a preferential direction of the detecting particle is present, such as WIMP (Sec. \ref{subsec:wimp}) or solar neutrino detection.   

\subsection{WIMP directional detection}
\label{subsec:wimp}
Dark Matter has emerged as a central topic in both particle physics and cosmology, representing a mysterious and yet-to-be-identified component of the Universe. Its existence finds strong support in astrophysical observations across various scales, such as discrepancies in galaxy rotation curves, gravitational lensing phenomena, and anomalies in galaxy clusters' velocity dispersions. These observations collectively point to the presence of Dark Matter, which dominates a considerable portion of the Universe's mass \cite{roos2010dark}. When assuming that Dark Matter consists of particles, one of the most interesting, testable, and theoretically motivated candidates are the Weakly Interacting Massive Particles (WIMPs). WIMPs are particles not predicted by the Standard Model (SM), but they fit well in beyond the Standard Model scenarios, such as Supersymmetric theories, as well as in the standard cosmological theory as relic matter from the early universe. WIMPs are expected to be electrically neutral, interact only gravitationally (or at most weakly) with ordinary matter, and have a lifetime comparable to the age of the Universe \cite{Roszkowski_2018}.\\
According to studies on our Galaxy’s rotation curves, the DM should form a halo that envelops the Galaxy, with DM particles moving following a Maxwellian velocity distribution. In this context, the Earth, which rotates around the center of the galaxy with a speed of about 220 km/s, toward the Cygnus constellation, experiences an apparent DM wind, due to its motion in the DM halo. The interaction of WIMPs from the halo with standard matter, due to the WIMPs mass ($\sim$ 1-100 GeV ), is thought to happen efficiently with atomic nuclei. Considering these mass ranges and velocities, the interaction of a DM particle with an atomic nucleus would produce a nuclear recoil of $\sim$ 1-100 keV \cite{Battat_2016}. Given the flux, the local DM density, and a cross-section of the order of the weak interaction, the expected interaction rate of DM below R $\sim$ 0.1 event/kg/y. These events need to be distinguished in a background of nuclear and electron recoils $\sim$ 10$^6$-10$^9$ times higher. To overcome this problem the experiments employ different techniques of particle identification and background rejection, based on the response of the detector to different particles, with the purpose of isolating an eventual DM signal. Moreover, dark matter experiments search for new signatures for positive dark matter identification.
The motion of the Earth around the Sun, and the motion of the Earth around the Galaxy center, across the DM halo with the Sun, gives two signatures for positive identification of DM. The first effect implies an annual modulation (few percent) of DM event rate, with a peak in the period of the year in which the Earth moves in the same direction as the Sun, and a trough when the Earth moves in the opposite direction. The second, much more robust effect, would imply an excess of nuclear recoil events in the direction of the Cygnus constellation in galactic coordinates.\\
Based on these last considerations, a directional DM detector able to measure the direction of nuclear recoil can be the key to positively identifying Dark Matter. Indeed with a directional detector, it will be possible to have a clear Dark Matter signal as a peak of events of nuclear recoil in the opposite direction of the Cygnus constellation over any possible background. This would be a signature that no background whatsoever can mimic. Finally, with a directional spectrum of nuclear recoils, the halo, the substructures of the DM halo, and the properties of DM as a particle can be studied \cite{Mayet_2016}.
CYGNO/INITIUM fits in this context aiming to perform directional dark matter searches thanks to its low threshold, and the capability to reconstruct the direction of interacting particles.
The main challenge for a directional DM experiment is to identify and reconstruct the direction of the very short track expected for a 1-100 keV nuclear recoil, long $\mathcal{O}$(nm) in solid, and $\mathcal{O}$(mm) in gas. To overcome this problem, directional detectors for DM are mainly gasseus Time Projection Chambers (TPCs).
In dark matter searches, moreover, the reduced mass WIMP-target system and the experimental energy threshold play a crucial role in defining the minimum DM mass to which an experiment is sensitive. Opting for a light target with atomic mass A < 10, coupled with a typical $\mathcal{O}$(1) keV energy threshold can potentially extend the experiment sensitivity to DM masses below 10 GeV, a portion of the parameter space that remains largely unexplored to date. For reduced mass reasons, the He used in the CYGNO gas mixture with $A=4$, lead to the maximization of the sensitivity to WIMP masses of a few GeV for SI couplings. Additionally, the favorable kinematic compatibility of He with WIMP of low mass, coupled with its light mass, results in longer NR produced after an interaction compared to heavier target elements, leading to better performances in the measurement of track directionality and head-tail recognition. Moreover, the abundant presence of fluorine atoms in CF$_4$ enables sensitivity to SD couplings, particularly at low WIMP masses close to the Fluorine mass. Consequently, thanks to its gas chemical composition, CYGNO stands out as one of the rare experiments in the DM detection field able at the same time to search both SI and SD interactions at low WIMP masses.
The low density of the gas has the advantage of a better track reconstruction, but it has the drawback of the lower mass-to-volume ratio.\\
A plot of the dark matter signature in galactic coordinates, as a dipolar angular distribution of wimp-NR, is shown in figure \ref{fig:wimpNRdistrib} for two different hypotheses of WIMP masses.
\begin{figure}
    \centering
    \includegraphics[scale=.4]{figures/WimpNRDistribution.png}
    \caption{WIMP calculated nuclear recoil distribution in galactic coordinates under the hypotheses of WIMP masses of 10 and 100 GeV respectively on left and right.}
    \label{fig:wimpNRdistrib}
\end{figure}
A Bayesian statistical analysis was conducted to assess the sensitivity of the CYGNO PHASE\_2 30 m$^3$ experiment in WIMPs detection in presence of background \cite{instruments6010006}. In this study, both direction and energy have been taken into account.
The sensitivity limits for both spin-dependent and spin-independent coupling interaction are shown in figure \ref{fig:SISDSensitivity} under different hypotheses of background level and threshold, for 3 years of exposure of a 30 $m^3$ experiment. The sensitivity limits with the addition of a Hydrogen-rich gas (iC$_4$H$_{10}$) have been evaluated.
\begin{figure}
    \centering
    \includegraphics[scale=.4]{figures/SensitivityCYGNODM.png}
    \caption{
The plots show the spin-dependent/spin-independent sensitivity for WIMP-proton cross sections in the 30 m$^3$ CYGNO detector over a 3-year exposure period. Different background level assumptions and operational thresholds of 1 keV (top plot) and 0.5 keV (bottom plot) are considered. The dashed curves represent scenarios with a number of background events (the number of background events) set at 100 (black), 1000 (red), and 10,000 (dark green). The dotted curves indicate the sensitivity for a He:CF$_4$:isobutane 58/40/2 mixture. Current constraints from PICO (purple) \cite{PhysRevD.100.022001}, DRIFT (orange) \cite{BATTAT201765}, and NEWAGE (cyan) \cite{10.1093/ptep/ptaa147} are also shown. The allowed region by DAMA \cite{PhysRevD.70.123513} is represented by the light green band, and the light gray dotted line represents the neutrino floor for C$_3$F$_8$, taken from PICO.}
    \label{fig:SISDSensitivity}
\end{figure}


\subsection{Migdal effect}
\label{subsec:migdal}
In the context of the "Framework per l’attrazione ed il rafforzamento delle eccellenze per la Ricerca in Italia" (FARE Ricerca in Italia), and in synergy with the INITIUM, ERC Consolidator Grant (Agreement N. 818744), the FINEM (Full Imaging of Nuclear recoils for Experimental Migdal measurement) aims to create a method for studying the Migdal effect using a high-precision gaseous Time Projection Chamber (TPC) with 3D optical readout. The Migdal effect, predicted in the Standard Model and first calculated by A. B. Migdal in 1941 \cite{Migdal1941}, has not been experimentally detected. It involves the potential for a recoiling atom to undergo rapid excitation or ionization during elastic scattering because the electron cloud does not immediately follow the recoiling nucleus. The electron cloud will follow the nucleus after a certain time, and in that time, with the displacement of positive and negative charges, a polarized state is created. With the relaxation of the polarized state, excitation or ionization can be induced within the recoiled atom through this process called Migdal. Although this effect has been widely employed by dark matter experiments to establish constraints \cite{Migdal1,Migdal2,Migdal3,Migdal4,Migdal5}, it has not yet been experimentally observed. Like in the search for dark matter, utilizing the Migdal effect in coherent neutrino-nucleus scattering can enhance the ability to detect solar neutrinos \cite{Ibe_2018}. Consequently, the experimental observation and measurement of the Migdal effect using FINEM can be considered of pivotal importance, benefitting both current and future efforts in dark matter research and solar neutrino spectroscopy. \\
The distinct Migdal signature appears as the simultaneous generation of a nuclear recoil and an ionization electron originating from the same point. This results from the elastic interaction between a neutral particle and a nucleus, as depicted in the left part of figure \ref{fig:MigdalSIgnature}. To experimentally observe this phenomenon, a detector must possess the capability to distinguish between these two distinct tracks, both originating from a shared source. Currently, the most suitable option for achieving this is a gaseous target, as it enables track lengths of the order of micrometers to millimeters, which are relevant for the energies of interest.
\begin{figure}
    \centering
    \includegraphics[scale=.45]{figures/MigdalSignature.png}
    \caption{Scheme of the Migdal effect signature. Left: In the first signature proposed the nuclear recoil is produced in coincidence with an electron recoil from a common vertex. Right: A second signature proposed from Migdal detection in which an X-Ray is produced from the primary vertex, and a second ER is found displaced from the main ionization cluster.}
    \label{fig:MigdalSIgnature} 
\end{figure}
From an experimental perspective, this detection strategy may face challenges when dealing with very low-energy nuclear recoils (NR) and ionization electrons, especially when high granularity Time Projection Chambers (TPCs) are employed (this also depends on the specific gas mixture used). To address this, a different approach was suggested in a previous study \cite{10.1093/ptep/ptaa162}, focusing on the concurrent emission of X-rays. This enables the additional electron recoil (ER) resulting from the X-rays to be spatially separated from the NR. In gases, an X-ray absorption length on the order of centimeters is expected. The Migdal process illustrating this concept is presented in the right part of figure \ref{fig:MigdalSIgnature} \cite{10.1093/ptep/ptaa162}. In this scenario, the NR and ionization electron are collectively detected as a single cluster A, while the X-ray, absorbed over a distance on the order of centimeters, appears as a distinct, monochromatic cluster B. It's important to note that this X-ray emission introduces an additional suppression factor (approximately 0.14 in Argon \cite{10.1093/ptep/ptaa162}), and not all atoms possess the electron shell configuration necessary for X-ray emission.
The FINEM project aims to develop a detector LIME-like, fine-tuning its design, operational parameters, shielding, and experimental arrangement within a neutron beam setup to investigate the Migdal effect using Ar/He:CF$_4$ gas mixtures. The choice of the neutron source is the Frascati Neutron beam facility, able to provide 14.1 MeV or 2.5 MeV neutrons with fluxes up to $10^{11}$ $10^{9}$ n/s respectively.
\begin{figure}
    \centering
    \includegraphics[scale=.5]{figures/ERNRMigdal.png}
    \caption{Left: Kinematic allowed region for Migdal. The x-axis refers to the energy of the nuclear recoil, while the y-axis refers to the ER energy. All the combinations of ER and NR energies below the curve are kinematically allowed. The different curves refer to different elements. Right: example of a Migdal event with signature \#1 in CYGNO.}
    \label{fig:ERNRMigdal}
\end{figure}
For a neutron flux of 14.1 MeV the kinematic allowed region is shown in figure \ref{fig:ERNRMigdal}, left plot. In more detail, given a nuclear recoil energy (x-axis) the y-axis shows the maximum allowed electron recoil energy. It can be observed that for a nuclear recoil of $100$ keV, very well detectable in CYGNO, an electron recoil up to several keV of energy can be produced from the same vertex. The right plot of figure \ref{fig:ERNRMigdal} shows how a Migdal event with signature \#1 would appear in CYGNO. The event has been produced with the CYGNO digitization algorithm (Chap. \ref{chap:Simulation}), and shows a 100 keV$_{ee}$ NR produced with a 30 keV ER with a common vertex. This track topology is very easy to distinguish from classical events given the very high-density energy release of the NR together with the curliness and peculiar energy release of the ER. A detailed study of the background of this process has been done for a low-pressure TPC similar to CYGNO. The number of background and signal events per million neutron-induced recoil tracks for 2.47 MeV and 14.7 MeV neutrons incident on CF$_4$ gas at 50 Torr has been evaluated and it results to be $\mathcal{O}(1)$, compared to a number of signal events $\sim$ 30 times higher.

\subsection{X-Ray polarimetry}
\label{subsec:polarimetry}

X-Ray polarization is a valuable observational method capable of shedding light on the emission mechanisms of exotic astrophysical phenomena characterized by strong gravitational and magnetic fields, intricate geometries, and explosive events \cite{marshall2020small}. It also holds the potential to enhance our understanding of solar flares and their implications in space weather science \cite{Fabiani:2011vr}. The limited progress of polarimetry in the X-ray energy range over the past four decades can be attributed to the absence of sufficiently sensitive instrumentation. Traditional techniques like Bragg diffraction (constrained by a narrow energy band) or Thomson scattering (inefficient for energies above 10 keV due to photoelectric absorption) were inadequate. Moreover, these techniques couldn't be easily integrated with X-ray optics, which restricted their application to just a few galactic sources. However, recent advancements in high-performance imaging and tracking devices have opened up new possibilities. Gas Pixel Detectors (GPDs) and Time Projection Chambers (TPCs), leveraging the photoelectric effect with the directionality power, have emerged as promising foundations for innovative and sensitive X-ray polarimeters \cite{articlePol1234,muleri2016performance,JKBlack_2007}.\\
In photoionization, the ionization process by means of a gamma interaction, the s-photoelectron is primarily emitted in alignment with the electric field of the incoming photon. This emission follows a probability distribution described by $cos^2(\vartheta)$, where $\vartheta$ is the polarization-dependent azimuthal angle with respect to the direction of the photon's momentum. Through the reconstruction of the photoelectron's impact point and its initial direction, a high-resolution gas detector has the capability to determine the linear polarization of X-rays. This measurement is achieved while retaining crucial information regarding the absorption point, energy, and timing of individual photons. Through the reconstruction of the photoelectron's impact point and its initial direction, a high-resolution gas detector has the capability to determine the polarization of X-rays. This measurement can be achieved while conserving essential information regarding the absorption point, energy, and timing of individual photons.\\
In recent years, the INAF research group involved in the HypeX project, in collaboration with a team from INFN Pisa, has pioneered the development of the first Gas Pixel Detector (GPD) designed for precise X-ray polarimetry measurements in a space environment \cite{FMuleri_2009}.
This GPD features a 1 cm drift distance Time Projection Chamber (TPC) filled with a He:DME gas mixture, single Gas Electron Multiplier (GEM) amplification, and an innovative charge pad readout system. The charge pad readout employs a finely subdivided custom VLSI ASIC created using 0.35 $\mu$m CMOS technology. This configuration enables full 2D imaging capabilities across a 15 x 15 mm$^2$ area, which is covered by 105,000 hexagonal pixels. The GPD can efficiently detect X-ray photoelectron tracks with energies of $\mathcal{O}$(10)keV, resulting from X-ray absorption.  
There are two main drawbacks to the use of the technologies developed up to now in the field of space polarimetry. The first one is that one class of detector used has a limited field of view and must be oriented toward the direction of the object to study. The second is that the TPC projected up to now are very small objects, and can measure the polarization of gammas in a range of a few keV.\\
In the context of CYGNO, the XRay-CMOS project, founded with a Progetto di Ricerca di Interesse Nazionale (PRIN), aims to develop a TPC with a large field of view for X-Ray polarimetry, in which there is no condition on the orientation of the incoming photon with respect to the detector drifting axis. 
To achieve this goal, the Xray-CMOS project will follow multiple lines, benefiting from the latest advancements in high-precision Time Projection Chambers (TPCs) for directional Dark Matter (DM) search experiments in various gas mixtures and innovative imaging techniques.
In particular, the project will specifically leverage the cutting-edge optical 3D readout method for Time Projection Chambers (TPCs), which has been recently pioneered by the CYGNO/INITIUM collaboration \cite{AbrittaCosta_2020,Baracchini_2020234,Baracchini_2020_Stab}. Employing CYGNO technology, a single sCMOS camera can cover an amplification region measuring 100$\times$100 mm$^2$, with each pixel capturing details within a 45$\times$45 $\mu$m$^2$ effective area. This represents a significant advancement, achieving almost two orders of magnitude improvement over the GDP detector, all while maintaining the same pixel dimensions. Moreover, with a detector of the size of MANGO at atmospheric pressure, ER can be detected with good directional performances within 10 to 60 keV. The performances in impact point and initial direction determination on low energy electron recoils will be discussed in Chapter \ref{chap:directionality}. The next steps for the development of the project will be the optimization of the gas mixture, eventually with the addition of SF$_6$, or other electronegative dopants. This will be followed by an optimization of the amplification structure, and finally the detector geometry for the specific X-ray polarimetry physics case.



\section{The CYGNO timeline}
\label{sec:Timeline}
The CYGNO project's final aim is to implement a large-scale detector for the directional detection of DM and Solar neutrino spectroscopy. To deeply understand and enhance the experimental technique, multiple prototypes have been developed. In figure \ref{fig:CYGNOTimeline} project's road map is shown.\\
\begin{figure}
    \centering
    \includegraphics[scale=.3]{figures/CYGNOTimeline.png}
    \caption{Timeline of the CYGNO experiment.}
    \label{fig:CYGNOTimeline}
\end{figure}
The initial prototype, ORANGE, consisted of a 10$\times$10 cm$^2$ area with a 1 cm drift gap, demonstrating the detection feasibility of O(1) keV energy deposits in the gas by coupling an sCMOS camera to a GEM amplification stage. Additionally, it evaluated the potential for 3D reconstruction by incorporating a PMT \cite{Campagnola:2313231}.
Following ORANGE, the subsequent prototype LEMOn featured a 20 cm drift gap and a more expansive readout area of 20$\times$24 cm$^2$. LEMOn was employed to investigate the detector's performance concerning a larger drift distance and readout area. In parallel, a prototype named MANGO, with a 10$\times$10 cm$^2$ readout area and an adjustable drift region, was built in 2018. MANGO's purpose was to conduct R\&D tests on different gas mixtures and amplification structures. In 2019, the construction of the LIME prototype concluded. LIME having a 50 cm drift and a 33$\times$33 cm$^2$ readout area detector represents the foundation for the larger-scale experiment. Following an overground commissioning phase, LIME was relocated underground at Laboratori Nazionali del Gran Sasso (LNGS) in June 2022 to undergo a comprehensive characterization of the detector in a future realistic environment. All these prototypes collectively constitute CYGNO PHASE\_0, aiming to affirm the optical readout's full capabilities using APS commercial cameras and PMTs, as well as validate the Monte Carlo simulation of anticipated backgrounds. Following PHASE\_0, the project advances to PHASE\_1, with a detector known as CYGNO-04, involving a 0.4 m$^3$ detector to be placed underground at the LNGS. This detector will embody all the technological and material selections envisioned for the forthcoming CYGNO-30. PHASE\_1 is designed to demonstrate the scalability of the experimental approach and the capabilities of the larger PHASE\_2 detector in achieving the anticipated physics objectives. Lastly, CYGNO-30, a detector of  $\mathcal{O}(30)$ m$^3$ in size, will mark the beginning of the project's PHASE\_2. An experiment of this scale, CYGNO-30, has the potential to make a substantial contribution to the investigation and understanding of Dark Matter (DM) with masses below 10 GeV, exploring both SI and SD couplings leveraging on the benefits of a directional search. 
Subsequent sections will delve into the latest prototypes and the primary results achieved with them.

%\subsection{Results from previous prototypes}

\section{The LIME prototype}
\label{sec:LIME}

The Long Imaging Module (LIME) is the largest prototype developed under the CYGNO experimental approach, representing a key milestone in the R\&D phase of the CYGNO project. A scheme of LIME is shown in figure \ref{fig:LimeScheme}. 
\begin{figure}
    \centering
    \includegraphics[scale=.4]{figures/LIMEScheme.png}
    \includegraphics[scale=.2]{figures/LIMEPic.png}
    \caption{Left: a scheme of the LIME prototype. Right: a picture of LIME}
    \label{fig:LimeScheme}
\end{figure}
The TPC has a rectangular-shaped sensitive volume, exhibiting a large readout area measuring 33$\times$33 cm$^2$ and a drift length of 50 cm, with a total active volume of 50 liters. These specific dimensions have been selected to replicate the drift length of the 0.4 m$^3$ CYGNO-04 detector (Sec. \ref{sec:CYGNOFut}). The external vessel is constructed from acrylic, ensuring durability and structural integrity. Additionally, an external Faraday cage, made of aluminum, shields the detector from any potential electromagnetic interference. Positioned at the top side of the vessel is a narrow opening that stretches along the drift distance, firmly sealed with a thin ETFE window. This design allows for the calibration of the detector using external radioactive sources since the window allows the passage of gammas. The cathode and the squared field rings that constitute the field cage are constructed from copper. The rings are positioned with a pitch of 16 mm and interconnected via ceramic resistors to create the voltage partitioning, for generating the drift field. The amplification stage relies on a triple stack of GEMs, each measuring 50 $\mu$m in thickness, with an area of 33$\times$33 cm$^2$. The GEMs are attached to an acrylic frame to minimize the radioactivity contribution. The GEM area is optically readout, employing a sCMOS camera and 4 PMTs placed at the 4 corners of the detector. This arrangement enhances PMT track reconstruction capabilities. The PMTs employed are of the Hamamatsu R7378A8 type, featuring a 22 mm diameter bialkali photocathode sensitive to wavelengths from 160 up to 650 nm. As for the sCMOS camera, the Hamamatsu ORCA Fusion (Table \ref{tab:cameras} for details) was used, along with a Schneider Xenon lens. The camera is positioned at approximately 62 cm distance from the closest GEM, and it images an area of 35.7$\times$35.7 cm$^2$. Consequently, each pixel within the 2304$\times$2304 pixel grid of the sCMOS sensor looks at an effective area of 155$\times$155 $\mu$m$^2$.

After a first phase of overground commissioning \cite{refId0}, LIME was transported and installed in the underground facility of the Laboratori Nazionali del Gran Sasso (LNGS), where it is currently operational in a low background environment. The primary objectives of LIME are validating the capabilities of the CYGNO approach within an underground setting, confirming the accuracy of Monte Carlo (MC) simulations to model the detector background, and testing both the construction and operational protocols for the realization of PHASE\_1 (Sec. \ref{sec:CYGNOFut}). Additionally, it will deliver a precise, spectral, and directional measurement of the environmental neutron flux at LNGS.

\subsection{LIME Overground commissioning}
Before its underground installation at the LNGS, LIME underwent a commissioning phase at the overground LNF. This step aimed to evaluate and document the studies on threshold, precise determination of absolute position along the drift direction, light output, and energy response. The subsequent section provides an overview of the results obtained during this commissioning phase.


%\subsubsection{Response to electron recoils}
%An initial standard assessment of the detector's response to energy releases around a few keV is accomplished using a $^{55}$Fe source featuring an activity of 115 MBq. The decay process of 55Fe involves electron capture, resulting in an excited $^{55}$Mn nucleus that subsequently emits X-rays at approximately 5.9 keV, accompanied by an additional emission around 6.4 keV.Due to the specific geometry of the source holder and trolley, the photon flux irradiates a cone with an opening angle of about 10 degrees. Consequently, in the central region of the detector, the photon flux is expected to exhibit a Gaussian transverse profile characterized by a standard deviation ($\sigma$) of roughly 1 cm as shown in figure \ref{fig:ironspotandprofile}.
%\begin{figure}
%    \centering
%    \includegraphics[scale=.35]{figures/IronSpot.png}
%    \includegraphics[scale=.6]{figures/TransvProf.png}
%    \caption{Left: picture of a 5.9 keV light spot from the $^{55}Fe$ source in LIME. Right: light profile of the iron spot projected on the x-axis.}
%    \label{fig:ironspotandprofile}
%\end{figure}
%Furthermore, to investigate the energy response concerning various X-ray energies, a compact multi-target source was utilized \cite{wheeler2018observation}. This source comprises a sealed $^{241}$Am primary source that is positioned in front of different materials selectively. Each material is presented one at a time to the primary source, causing its characteristic X-rays to be emitted through a 4 mm diameter aperture.Additionally, considering the significance of understanding the detector response at low energies, X-rays from the $^{55}$Fe source with an energy of approximately 6 keV were employed to stimulate the emission of X-rays with lower energies in two other materials: titanium (Ti) and calcium (Ca). Due to the experimental arrangement used to excite the Ti and Ca lines, the 6 keV X-rays from the $^{55}$Fe source can also enter the active volume of the detector, resulting in the overlapping of both contributions. A detailed description of the analysis and results of this study is given in chapter \ref{ch:XRayAn}.


\subsubsection{Characterization of $^{55}$Fe signal}
The $^{55}$Fe source produces gammas which, as reported in figure \ref{fig:Fexydistrib}, interact in the gas mixture, illuminating the entire vertical size of the detector. However, due to source collimation, only a narrow region in the horizontal direction exhibits notable occurrences of $^{55}$Fe-induced clusters.
\begin{figure}
    \centering
    \includegraphics[scale=.3]{figures/55FeXYDistrib.png}
    \caption{X-Y distribution of the reconstructed $^{55}Fe$ cluster. The source, as can be noticed is positioned out of the detector at high y values.}
    \label{fig:Fexydistrib}
\end{figure}
Multiple parameters are employed to characterize these tracks, including $\sigma_T$ (representing the track length), $\delta$ (a measure of light density defined as the integral of the collected light in the cluster divided by the number of pixels above the noise threshold), and the RMS of the light intensity residual across the pixels $I_{rms}$, and other quantities described in \cite{Baracchini:2020nut}. 
A $^{55}Fe$ cluster sample is obtained using a loose selection on the total dataset. The resulting distributions of $\delta$ and $\sigma_T$ for the clusters passing the selection are shown in figure \ref{fig:55feselected}, where additionally to the data acquired with the $^{55}Fe$ source also the plots for natural radioactivity and pedestal are shown. 
\begin{figure}
    \centering
    \includegraphics[scale=.5]{figures/deltasigmaIron.png}
    \caption{In figure, the distribution of light density and sigma of the transverse profile of the track, respectively left and right plot, are shown for run with $^{55}Fe$ source, without source, and for noise run.}
    \label{fig:55feselected}
\end{figure}
Additionally, the distributions of the $I_{sc}$, defined as the sum of the detected light within a cluster, are shown for very low energies and around the $^{55}Fe$ peak in figure \ref{fig:scIntegralFE}.
\begin{figure}
    \centering
    \includegraphics[scale=.5]{figures/sc_integralFe.png}
    \caption{In figure, the light integral distribution for a low energy region and for the region around the 5.9 keV peak, respectively left and right plot, are shown for run with $^{55}Fe$ source, without source, and for noise run.}
    \label{fig:scIntegralFE}
\end{figure}
The I$_{sc}$ distribution shows a second bump at approximately twice the expected energy from $^{55}$Fe X-rays. This happens because two adjacent 5.9 keV spots might be merged into a single light cluster with energy double that of a single light spot. Such occurrences are attributed to the relatively high activity of the employed $^{55}$Fe source. 
The distributions represent the dataset acquired, both with and without the X-ray source. In this way, the background contribution can be studied by normalizing the background data to the live-time of the data collected with the $^{55}$Fe source. An estimation of the contribution from random clusters, defined as clusters formed by chance from neighboring pixels exceeding the zero-suppression threshold was derived from the pedestal runs, where no signal contribution of any kind is expected. As can be seen from figure \ref{fig:scIntegrwalFE} left, this contribution became negligible when $I_{sc}$ exceeds 400 photons. 

\subsubsection{Spatial Dependencies in light yield measurement}
The light yield measured for a cluster is still influenced by the location of the initial ionization event within the active volume where the interaction occurred. Consequently, it is necessary to convert the light yield $I_{sc}$ into an energy value E$_{rec}$ using a calibration factor, and subsequently, correct it to estimate the original energy deposition E. \\
The relationship between E$_{rec}$ and the x-y coordinates of the initial interaction may be influenced by various factors, including potential issues in correcting for the vignetting effect, non-uniformities in the drift and amplification fields, particularly near the edges of the GEM planes, as illustrated in figure \ref{fig:xylightFe} left plot.
\begin{figure}
    \centering
    \includegraphics[scale=.5]{figures/ResponseVsXYZ.png}
    \caption{Left: total light integral as a function of the position on the x-y plane with the detector illuminated by the $^{55}$Fe source. Right: Position of the iron peak normalized to its value @25cm as a function of the distance of the source.}
    \label{fig:xylightFe}
\end{figure}
Furthermore, inefficiencies in the transport of primary ionization electrons caused by attachment during their drift in the gas, are expected to lead to a consistent reduction in $I_{sc}$ with respect to the z-coordinate of the initial interaction. However, as depicted in Figure \ref{fig:xylightFe} right plot, there is a continuous increase in $I_{sc}$ as a function of the z-coordinate of the initial interaction.\\
This phenomenon can be explained as follows: during the amplification process, ions and electrons generated in the avalanches fill the holes on the GEM foils. While the holes small size allows them to quickly leave the amplification region, in \cite{7581778} it has recently demonstrated that for high-gain operations (in the range of 10$^6$ to 10$^7$), the charge produced by a single avalanche is already significant enough to locally alter the electric field. Typically, this has the effect of reducing the effective GEM gain, leading to a saturation phenomenon. This leads to a GEM system response that relies on the quantity of charge entering the single channels. Thus in case of longer tracks, this effect is strictly influenced by the local charge density along the track. In the context of LIME, the primary ionization electrons diffuse across the 50 cm drift path both transversely and longitudinally. The diffusion process significantly increases the region of volume containing the primary electron involved in the amplification process. As a result, the diffusion, reduces the charge density, mitigating the impact of gain reduction.\\



\subsubsection{Absolute z position}
The capacity to reconstruct the three-dimensional spatial positions of events within the detector enables, as demonstrated in previous research \cite{Brack_2014}, the rejection of events occurring near the sensitive volume's edges, likely originating from radioactivity within the detector materials (e.g., GEM, cathode, field cage).
As shown in other studies, the optical readout provides submillimeter accuracy in reconstructing spot positions within the x-y plane \cite{Antochi_2018,Marafini_2015}. To determine the z coordinate, the effects of electron diffusion during the drift path in the gas, well known, can be used. 
Exploiting this principle, a straightforward method was developed for ultra-relativistic particle tracks \cite{ANTOCHI2021165209}, relying on the standard deviation of the Gaussian which fit the track transverse profile.
With LIME, the assessment of z-reconstruction performance involves the examination of various shape variables associated with the spots generated by the $^{55}Fe$ source. This analysis is conducted by studying the behavior of several shape variables of $^{55}Fe$ spots varying the z coordinates of the source. The parameter that exhibited better performance, denoted as $\xi$, is determined by the product of the Gaussian sigma, $\sigma_{tr}$, fitted to the transverse profile of the spots, and the standard deviation of the counts per pixel within the spots, $I_{rms}$. In figure \ref{fig:xivsz}, it can be seen the distribution of $\xi$ for all reconstructed spots as a function of the nine distinct $^{55}Fe$ z values, ranging from 5 cm to 45 cm. For each z value, the mean value of the $\xi$ distribution is depicted, and a quadratic fit is also applied to illustrate the relationship between these average values and the z position of the source.
\begin{figure}[h]
    \centering
    \includegraphics[scale = .5]{figures/XiVsZ.png}
    \caption{In figure the $\xi$ distributions as a function of the z position of the $^{55}Fe$ source are shown (gray bands). The mean values of the distributions (blue dot) fitted with a quadratic equation (black line) are also present together with the result of the fit. }
    \label{fig:xivsz}
\end{figure}
As observed in the figure, there are evident tails in all instances. However, the core of the spots distributions exhibit increasing $\xi$ values as z increases. In figure \ref{fig:xivszres}, plot on the left, the distribution of the z residuals for clusters reconstructed using the measured $\xi$ values, at a fixed $^{55}Fe$ z position of 20 cm is shown. 
\begin{figure}[h]
    \centering
    \includegraphics[scale=.35]{figures/XiVsZRes.png}
    \includegraphics[scale=.45]{figures/ResidualTrend.png}
    \caption{Left: distribution of the z residuals for clusters reconstructed using the measured $\xi$ values for the $^{55}Fe$ position z=20 cm. Right: trend of the $\Omega$ parameter for different z values with superimposed a linear fit.}
    \label{fig:xivszres}
\end{figure}
The residual distribution has been modeled using a Novosibirsk function \cite{bukin2007fitting} and, from this fit, the parameter $\Omega$ (representing the FWHM/2.36) is derived. In the same figure \ref{fig:xivszres}, plotted on the right, the $\Omega$ values obtained from the nine datasets at the different z positions are also presented.
It's noteworthy to notice that even for events occurring near the cathode, this method demonstrates the capability to estimate the z position of interactions involving $^{55}Fe$ photons with an uncertainty of less than 10 cm, despite a slight worsening in the absolute uncertainty as the spots move farther away from the GEM.

%\subsubsection{Stability of detector operation}
%Dark Matter (DM) searches necessitate of extended periods of data collection, spanning months or even years. This requires ongoing monitoring of the detector's performance to ensure stability. In the case of the LIME prototype, its stability has been assessed by continuously operating the detector for a period of two weeks at the Laboratori Nazionali di Frascati (LNF). During this period, data were acquired automatically, including runs of pedestal events and 55Fe source runs. In this, period of time no issues were reported in writing data apart from a couple of instances where data couldn't be saved due to issues with the laboratory's internal network. The laboratory maintains a heating system to regulate temperature, resulting in a relatively stable room temperature with an average value of $298.7 \pm 0.3$ K during the testing period. Meanwhile, atmospheric pressure exhibited visible fluctuations, with a significant oscillation of approximately 22 mbar in the later stages of the test, as shown in figure \ref{fig:AtmPressure}.
%\begin{figure}
%    \centering
%    \includegraphics[scale=.4]{figures/AtmPressure.png}
%    \caption{Behaviour of the atmospheric pressure in LIME room as a function of the time}
%    \label{fig:AtmPressure}
%\end{figure}
%The average number of photons in the spots resulting from $^{55}$Fe X-ray interactions has been also assessed. The behavior of this quantity, normalized to its initial value, is presented in the left plot of figure \ref{fig:FeVariation}.
%\begin{figure}
%    \centering
%    \includegraphics[scale=.4]{figures/LightVariation55Fe.png}
%    \caption{Left: Plot of the light output at 5.9 keV as a function of the elapsed time. The values are normalized at the light yield at t=0. Right: Plot of the light output at 5.9 keV as a function of the atmospheric pressure in LIME room. The values of light output are normalized to the same value at t=0 of the plot on the left.}
    \label{fig:FeVariation}
%\end{figure}
%The light yield of the detector exhibited a nearly constant increase throughout the data collection period. This observed trend can be directly associated with fluctuations in gas pressure, as illustrated in the right part of figure \ref{fig:FeVariation}. Through a linear fit of the data, we determined that the light yield decreased by approximately 0.6\% per millibar. This decrease is attributed to the anticipated reduction in gas gain as the gas density increases, in agreement with \cite{blum2008particle}. At the moment, systematic measurements to correct the effect of temperature, pressure, and humidity on the detector light yield are in progress.

\subsection{ER/NR discrimination}
The capability to distinguish nuclear recoil and electron recoil is of fundamental importance for dark matter searches. Indeed low energy electron recoil in CYGNO can mimic a neutron/WIMP interaction at very low energies. Thanks to the high granularity TPC approach, it is possible to use a large amount of information on the track to efficiently discriminate between NR and ER.
To assess the capability of ER/NR discrimination a smaller CYGNO prototype, named LEMOn, featuring a 20 cm drift length and a 24$\times$20 cm$^2$ readout area, has been exposed to $^{55}Fe$ source and $^{241}$AmBe source producing neutrons. The detector was shielded with lead in order to minimize the contribution from external gamma.
The measurement has been performed overground at Laboratori Nazionali Frascati. This implied a high occupancy of cosmics rays in the tracks among which the interesting events must be found. To discriminate the interesting events of $^{55}Fe$ spots and nuclear recoil from, cosmics and high-energy electrons the shape variables of the tracks have been used. Of particular relevance are the track length and the track slimness (ratio length/width) which can be used to separate short and round tracks from extended tracks. The former tracks indeed appear as a round, thick, and dense light spot, while the latter, with a much lower energy ionization profile, appear as long and slim tracks.
What mainly discriminates ER and NR is the energy ionization profile $dE/ dx$. This second category of tracks has a much higher $dE/ dx$. 
A variable called light density $\delta$, proportional to the $dE/ dx$, and defined as the total number of photons in the cluster divided by the total number of pixels can thus be employed to discriminate ER and NR. 
As can be seen from the left plot of figure \ref{fig:ERNRDiscr} the light density variable can be obtained to separate the NR from the $^{241}$AmBe run and the ER from the $^{55}Fe$ run. In particular with two different selections on $\delta$ considered, $\delta>10$ and $\delta>11$ an efficiency in background rejection respectively of 96\% and 99\% can be obtained while keeping an efficiency on the signal of 50\% and 40\% respectively.
\begin{figure}
    \centering
    \includegraphics[scale=.4]{figures/ERNRDiscrimination.png}
    \caption{Left: distribution of the delta variable for background run, $^{241}$AmBe run and $^{55}Fe$ run. The scale factors on the distributions are for live-time normalization purposes. Right: plot of the signal efficiency as a function of the energy for the two different cut $\delta>10 / 11$ with efficiency on background identification of $4-1\%$ respectively.}
    \label{fig:ERNRDiscr}
\end{figure}
\cite{Baracchini:2020nut}
The same efficiency has been computed for the two $\delta$ selections as a function of visible energy, and the results are reported in the right plot of figure \ref{fig:ERNRDiscr}. This measurement highlights the discrimination capability of the TPC optical approach. Despite the selection cut used being very loose and basic, a rejection power of $\sim 10^2$ can be reached below 10 keV. A multivariate analysis based on machine learning techniques for ER/NR discrimination is in progress and could exploit the full topological information to improve CYGNO discrimination capabilities.

\subsection{LIME Underground}
One of the primary objectives of the LIME prototype is to evaluate its performance in the low-background environment of the Laboratori Nazionali del Gran Sasso (LNGS), where it has been in operation since June 2022. The experimental setup is situated in a container positioned within the corridor between Hall B and Hall A, directly in front of the DAMA/LIBRA experiment. The container spans two levels: the lower floor houses the detector and any future shielding, while the upper floor accommodates the control room, which also houses the data acquisition (DAQ) servers, modules, and high-voltage supplies. In figure \ref{fig:LimeUndergr}, two images of the underground LIME site are shown. The gas system is located just outside the experimental area and is provided by an Air Liquide GAS system. This system manages the mixture's flow to the detector, purifies it from impurities, recirculates it, and facilitates the recovery for the disposal of greenhouse gases.
\begin{figure}
    \centering
    \includegraphics[scale=.4]{figures/LIMEUnderground.png}
    \caption{}
    \label{fig:LimeUndergr}
\end{figure}

\subsubsection{Background studies and underground program}
\label{sec:bkgStudies}
Understanding and characterizing the radioactive background is of paramount importance, particularly when searching for rare events. To address this, a comprehensive Monte Carlo (MC) simulation of the expected background in LIME was conducted using the GEANT4 software\cite{AGOSTINELLI2003250}. This simulation incorporated the CAD engineering design of the prototype, including various shielding configurations. The external radioactive background, originating from sources outside the detector, was simulated using neutron and gamma flux spectra measured at the Gran Sasso National Laboratory (LNGS) by other experiments \cite{DEBICKI2009429,Belli1989DeepUN}. The radioactivity of the detector components used to build LIME, which includes cathode, copper shielding, field rings, resistors, GEM, acrylic vessel, camera lens, and body, has been measured from the LNGS low radioactivity laboratory with a high purity Germanium detector, and the results have been used for the internal radioactivity simulation. \\
%In the unshielded setup, which includes only the Faraday cage, the dominant source of background radiation is from external factors, resulting in approximately 10$^9$ events per year above 1 keV, equivalent to a rate of about 36 Hz. To optimize the shielding configuration, a cost-benefit analysis was conducted with the objective of reducing the external background contribution while keeping costs to a minimum. This assessment considered factors like available space and the additional radioactive contribution introduced by the shielding materials. Ultimately, the most cost-effective solution identified was to utilize a 10 cm thick copper shield, encased within a 40 cm thick water tank shield. The copper portion of the shield effectively stops all $\beta$ decays and significantly reduces gamma radiation. Conversely, water is employed to moderate and stop neutrons due to the abundant hydrogen content in the liquid. This shielding configuration is found to result in fewer than 2 nuclear recoils (NRs) per year above 1 keV induced by external background in the active detector volume, while electron recoils (ERs) are expected to be reduced to 10$^5$ per year in the energy range of 1 to 20 keV.
The simulated energy spectrum of total recoils induced by internal radioactivity is presented in figure \ref{fig:ERNRBackground} left plot, while the nuclear recoils spectrum is presented in figure \ref{fig:ERNRBackground} right plot. Different colors represent the contributions from each detector component considered in the simulation. Notably, the field rings, resistors, and GEMs are among the primary contributors to the radioactivity budget, with a significant impact also observed from the camera lens and body. Addressing which are the most radioactive materials is crucial for future detector development.
\begin{figure}
    \centering
    \includegraphics[scale=.5]{figures/ERNRBackgroundSpectrum.png}
    \caption{Left (Right): ER+NR (NR) spectrum induced in the detector from the different detector components. Plots by Flaminia Di Giambattista.}
    \label{fig:ERNRBackground}
\end{figure}
%By implementing geometrical cuts within the detector volume-specifically, 1 cm from the borders and GEMs in the x-y plane, and 4 cm from the cathode in the z direction- the recoil events induced by background sources can be significantly reduced. This results in a 96\% reduction for electron recoils (ERs) and a 99.97\% reduction for nuclear recoils (NRs). With these initial cuts applied, the total number of recoils below 20 keV decreases to approximately 2.7$\times$10$^5$ events per year, with only 6 of them being NRs.
This analysis has been conducted using real events simulated without accounting for detector performance. The collaboration is actively working to incorporate the detector's response and refine the analysis strategy and selection criteria. 
%An overview of the annual contributions of internal and external electronic recoils (ERs) and nuclear recoils (NRs) in the different shielding configurations, taking into account fiducial cuts. 
%Initial images acquired with LIME in the underground site, featuring only the Faraday cage, indicate a recoil rate of approximately 35 Hz, which aligns with the anticipated value from the simulation.
The underground installation and operation of LIME has several purposes, including background studies, the validation of MC simulations, and neutron flux measurements. As each of these goals necessitates different configurations and background levels, the underground LIME program will be implemented in a phased manner, with additional shielding layers progressively added around the detector. The planned phases include:
\begin{outline}
    \1 Run0 No shield: 
        \2 Operation with LIME in the Faraday cage. 
        \2 Characterize the response of the detector underground and study the external background. 
        \2 Test on the control and DAQ system. Data-MC first comparison.
    \1 Run1 4cm Cu:
        \2 Study the impact of 4 cm Cu on the background.
    \1 Run2 10cm Cu:
        \2 Final copper shielding configuration with gamma suppression factor $10^3$.
        \2 Perform a spectral and directional measurement of neutron flux at LNGS to renew old measurements \cite{DEBICKI2009429,Belli1989DeepUN,Bruno_2019}
        \2 Perform a measurement with neutrons from $^{241}$AmBe.
    \1 Run2 10cm Cu + 40 cm water:
        \2 Strongly suppress the external neutrons
        \2 Internal radioactivity dominant contribution
        \2 Background data acquisition to study in detail the internal radioactivity
        \2 Comparison with the MC
\end{outline}
A summary of the annual internal and external contributions of ERs and NRs in different shielding configurations described for the different runs, comprising fiducial cuts is presented in table \ref{tab:bkgcontrib}. Initial images captured by LIME at the underground site with only the Faraday cage indicate a recoil rate of approximately 35 Hz, aligning well with the anticipated value from the simulation.

\begin{table}[!ht]
    \centering
    \scalebox{0.8}{
    \begin{tabular}{|l|ll|ll|ll|}
    \hline
        Shield &  Internal & ~ &  External & ~ & Total ~ & \\ 
        ~ & ER/y & NR/y & ER/y & NR/y & ER/y & NR/y \\ \hline
        No shield  & 1.13$\times$ 10$^9$ & 1450 & 7.26$\times$ 10$^6$ & 6.11$\times$ 10$^4$ & 1.14$\times$ 10$^9$ & 6.25$\times$ 10$^4$ \\ \hline
        4 cm Cu & 2.64$\times$ 10$^7$ & 850 & 7.26$\times$ 10$^6$ & 6.11$\times$ 10$^4$ & 3.43$\times$ 10$^7$ & 6.19$\times$ 10$^4$ \\ \hline
        10 cm Cu & 1.95$\times$ 10$^6$ & 915 & 7.26$\times$ 10$^6$ & 6.11$\times$ 10$^4$ & 9.78$\times$ 10$^6$ & 6.20$\times$ 10$^4$ \\ \hline
        10cm Cu + cuts & ~ & 772 & ~ & 16 & ~ & 778 \\ \hline
        40 cm H$_2$O + 10 cm Cu & 5.09$\times$ 10$^5$ & 2 & 7.26$\times$ 10$^6$ & 6.11$\times$ 10$^4$ & 8.34$\times$ 10$^6$ & 6.11$\times$ 10$^4$ \\ \hline
        40 cm H$_2$O + 10 cm Cu + cuts  & 2.0$\times$ 10$^4$ & 2 & 2.8$\times$ 10$^5$ & 17 & 3.3$\times$ 10$^5$ & 19 \\ \hline
    \end{tabular}
    }
    \caption{}
    \label{tab:bkgcontrib}
\end{table}

\section{Parallel research lines with the MANGO prototype}
\label{sec:MANGO}
The Multipurpose Apparatus for Negative Ion Studies with GEM Optical Readout (MANGO) is a compact detector featuring a 10$\times$10 cm$^2$ amplification area and an adjustable drift region \cite{Baracchini_2020EL}. MANGO fits in the CYGNO context as an experimental platform for different purposes, including testing different amplification systems and gas mixtures, testing the electroluminescence for enhanced light production in a CF$_4$ based gas mixture, and investigating the feasibility of negative ions operation with optical readout.\\
The amplification stage is constructed using a series of GEMs, each measuring 10$\times$10 cm$^2$, and spaced 2 mm apart, with a transfer field of 2.5 kV/cm applied between the GEMs. MANGO is typically equipped with triple 50 $\mu$m thin GEMs, although various thicknesses and stacking configurations have been subjected to testing (Sec. \ref{sec:gemgasmix}). The GEMs are labeled from 1 to 3, with GEM1 positioned closest to the drift region. These GEMs are supplied power by the HVGEM, a customized high-voltage source developed by the Laboratori Nazionali di Frascati (LNF). The HVGEM serves as an active high-voltage divider and is designed to provide power to seven separate and independent channels (3 GEMs + 1 cathode). Additionally, positioned at a distance of $\Delta$z = 3 mm from the main setup, there is a metallic mesh adopted from an ATLAS MicroMegas. This mesh, comprising 30 $\mu$m diameter metallic wires at a 50 $\mu$m pitch, yields a transparency of approximately 0.55 and is strategically placed to induce an electric field beneath the electrode of the last GEM amplification stage. In the last studies, the metallic mesh was substituted with an ITO glass, which features a higher transparency of 0.9.\\
MANGO is commonly operated in continuous gas flow mode and is housed within a light-tight enclosure made of 3D-printed black plastic. This enclosure contains an airtight acrylic vessel that holds the gas. A slim, highly transparent (transparency $>$ 0.9) Mylar window isolates the gas detector from the optical readout system. The light is readout by an Orca Fusion sCMOS camera \ref{sec:camera} and a PMT Hamamatsu H3164-10 \cite{PMTMAN}. The optical readout components are positioned at a distance of (20.5 $\pm$ 0.3) cm and are focused on the closest GEM plane. The camera is coupled to the detector and isolated from the light through an adaptable bellow. In this configuration, the camera images an area of approximately 11.3$\times$11.3 cm$^2$, leading to an effective pixel size of around 49$\times$49 $\mu$m$^2$. A scheme of the MANGO detector is shown in figure $\ref{fig:MANScheme}$
\begin{figure}
    \centering
    \includegraphics[scale = .3]{figures/MANGO_Scheme.png}
    \caption{Scheme of the mango detector. The sensitive volume (A), the adaptable bellow (B), and the CMOS camera (C) are shown. In the square, a scheme of the TPC with the cathode and the three GEMs is shown.}
    \label{fig:MANScheme}
\end{figure}

\subsection{Test on different GEMs configurations and gas mixture}
\label{sec:gemgasmix}
A comprehensive study of the detector performance involving various He:CF$_4$ gas mixture ratios (e.g., 60/40, 70/30) and different GEM thicknesses and stacking configurations is conducted. Two categories of GEMs have been utilized: one featuring thin 50 $\mu$m GEMs with 70 $\mu$m radius holes and 140 $\mu$m pitch (referred to as "t"), and the other consisting of thicker 125 $\mu$m GEMs with 175 $\mu$m radius holes and 350 $\mu$m pitch (referred to as "T"). All measurements are conducted under atmospheric pressure conditions at the Laboratori Nazionali del Gran Sasso (LNGS), situated at an elevation of approximately 1000 meters above sea level (a.s.l.), which corresponds to a pressure of (900 $\pm$ 7) mbar. In these studies, a $^{55}$Fe X-ray source with an activity of approximately 480 kBq is utilized to produce 5.9 keV electrons within the active gas volume of the MANGO detector. The relatively low source activity enables the reconstruction of each individual $^{55}$Fe track in the sCMOS images. 
The light spectrum of the reconstructed events is fitted with a Gaussian function, and the fitted mean value is considered as the light integral. The light integral as a function of the total voltage applied to the GEM is shown in figure \ref{fig:LightVsV}
\begin{figure}
    \centering
    \includegraphics[scale=.35]{figures/LightVsV.png}
    \caption{In figure the light integral as a function of the total voltage applied to the GEM for different GEMs stacking configuration and gas mixture is shown}
    \label{fig:LightVsV}
\end{figure}
Each set of GEM stacking configurations (i.e., ttt, Tt, and TT) exhibits a consistent gain slope. In contrast, the helium to CF$_4$ ratio affects the voltage required on the GEMs to achieve a similar gain, with a higher helium content allowing for lower voltages. The total achievable light output remains within the same order of magnitude for the same amplification structure. The highest gain and light output are attained with the three thin GEM configurations (ttt), with integral values averaging about three times higher than Tt and up to approximately five times higher than TT. From the $\sigma$ of the Gaussian used to fit the $^{55}Fe$ peak, the energy resolution at 5.9 keV has been studied in the different configurations. The energy resolution, defined as the ratio $\sigma$/mean, as a function of the total GEM voltage applied is shown in figure \ref{fig:EresoIron}
\begin{figure}
    \centering
    \includegraphics[scale=.45]{figures/EResoIron.png}
    \caption{The energy resolution at 5.9 keV as a function of the total voltage applied to the GEMs for different configurations is shown.}
    \label{fig:enter-label}
\end{figure}
An analysis of the $^{55}$Fe spots in the gas also allows for a measurement of the contributions from the amplification stage to overall track diffusion. This has been measured as a function of the total GEM voltages and considering all the possible combinations of GEMs and gas mixtures. The diffusion has been measured by fitting with a Gaussian the projection on x and y of the light contained in the iron spot. The final value of the sigma has been obtained by averaging these quantities. The results are shown in figure \ref{fig:diffsigmaFe}.
\begin{figure}
    \centering
    \includegraphics[scale=.35]{figures/SigmaFestud.png}
    \caption{In figure the average sigma of the iron spots as a function of the different GEM voltages for the different configurations is shown. }
    \label{fig:diffsigmaFe}
\end{figure}
From the plot, it can be observed that as expected the configurations with two amplification stages perform better in diffusion with respect to the one with 3 GEMs. This confirms the assumption that each stage contributes independently to the total diffusion. Another enforcement of this argument is that the diffusion with two GEMs is around 2/3 of the one with 3 gems.
Moreover, the Tt configuration performs better than the TT due to the closer hole pitch of t GEMs. Indeed the t GEM has a hole pitch of 140 $\mu$m while the T one has a pitch of 350 $\mu$ m. The camera, with a granularity of 49$\times$49 $\mu$m$^2$ seen by each pixel, is indeed sensible to this feature. 

\subsection{Electroluminescence studies}
Considering the significance of increasing light yield in optically readout TPCs (Sec. \ref{sec:camera}) a detailed analysis of the impact of a strong electric field applied in the induction region has been analyzed. As discussed in Sec. \ref{sec:gasmixture} there is the possibility to trigger the release of visible photons through the fragmentation of CF$_4$ into neutral CF$_3*$ without generating additional electrons. To explore this potential, an induction field ($E_{Mesh}$) is implemented in the induction region under the final GEM electrode. This field has been applied with the use of an ITO powered with a positive tension. The gain in light is examined across various GEM stacking configurations and gas mixtures, and the variation in light gain due to changes in the induction field is consistent across all the stacking configurations and gas mixtures investigated. The relative light yield increase as a function of the drift applied is shown in figure \ref{fig:Electrolum}
\begin{figure}
    \centering
    \includegraphics[scale=.45]{figures/Electroluminescence.png}
    \caption{In figure the light as a function of the induction field for different configurations is shown.}
    \label{fig:Electrolum}
\end{figure}

\subsection{Negative ions drift studies}
\label{sec:NID}
One significant limitation of large gaseous TPCs is that the electron cloud, drifting to the amplification plane, often degrades the intrinsic characteristics of the initial ionization track created by the particle interacting with the gas, mainly due to diffusion. There are two main contributions to the diffusion: one occurring during the particle's drift within the sensitive TPC volume and the other during the subsequent amplification processes. A method used to reduce transverse diffusion (along the GEM plane) is to apply a uniform magnetic along the drift direction \cite{blum2008particle}. Instead, the potentiality to decrease the diffusion by introducing a small percentage of SF$_6$ to switch to negative ions drift operation has been studied with the MANGO detector in the context of the INITIUM (Innovative Negative Ion TIme projection chamber for Underground dark Matter searches) project. This enables the creation of more compact detectors featuring longer drift distances, which leads to an improvement in tracking capabilities compared to electron drift (ED) operations. Moreover, it offers advantages in terms of volume scalability and reduced background contamination. Typically negative ions have been employed at low pressure ($<$100 tor), with few exceptions close to the atmospheric pressure \cite{Baracchini_2018NID,LIGTENBERG2021165706}, but never with optical readout.

\subsubsection{Negative ion drift operations}
The addition of an electronegative species to the gas mixture has the potential to modify the characteristics of the gas, thereby modifying the traditional operation of a Time Projection Chamber \cite{Martoff:2000wi,Ohnuki_2001}. Specifically, free electrons can be promptly captured by these electronegative dopants, typically in the range of distances of $\mathcal{O}$(10 $\mu m$), resulting in the formation of negative ions. Guided by the applied electric field, these anions drift towards the anode, assuming the role of effective charge carriers in place of electrons. Upon reaching the anode, the intense electric fields stimulate the release of the additional electron, initiating a standard electron avalanche. This modified TPC operation offers two key advantages: a reduction in diffusion, leading to better tracking performances, and the ability to fiducialize the detector.\\

\textbf{Diffusion reduction} A key benefit of Negative Ion Drift (NID) operation is the minimized diffusion during the drift. This is because the diffusion coefficient is directly proportional to $\sigma_T\propto\sqrt{\bar{E}}$, where $\bar{E}$ is the average energy of the drifting particle \cite{blum2008particle,Ohnuki_2001}. Electrons are significantly lighter than gas molecules by orders of magnitude $>10^4$, leading to an inefficient momentum transfer during collisions. Consequently, when electrons experience collisions with ions, their outgoing direction is randomized, and they preserve most of the kinetic energy acquired from the electric field in the time between two consecutive collisions. Conversely, the anion masses are comparable to the one of the gas molecules, enabling them to thermalize and disperse the energy acquired from the drift field in an efficient way. By employing this approach, diffusion can be minimized to the thermal limit \cite{blum2008particle}, resulting in diffusion orders of magnitude smaller \cite{DRIFT:2014bny}. The approximate formula in the low field limit describing the transversal diffusion $\xi$ of a charged cloud traveling a distance $L$ under the influence of an electric field $E$ is
\begin{equation}
    \xi^2 = \frac{2k_BT_{eff}L}{eE}
    \label{eq:diffequation}
\end{equation}
where $k_B$ is the Boltzmann constant, $T_{eff}$ is the temperature of the gas in Kelvin, and $e$ is the electric charge. Minimizing diffusion significantly enhances directional capabilities and background rejection, as the track topology is less affected by charge dispersion. The maximum drift length in a Time Projection Chamber, essential to increase the detector mass without increasing the detector complexity, is directly linked to diffusion properties. At greater distances, the smearing effect becomes pronounced, causing all track types to appear as blurred, large spots. Negative ions can therefore allow for an increase in the field cage length of the detector without compromising performance compared to regular Electron Drift (ED) operations.\\

\textbf{Fiducialization} The fiducialization refers to the capability to identify the 3D position of an event in a detector. In a TPC featuring an optical readout, the most challenging position to measure is along the drift direction $z$. Through Negative Ion Drift (NID) operation, it has been proven that multiple species of negative ion carriers, each with different masses, can be generated in the primary electrons capture process \cite{Snowden-Ifft:2013vua}. Among these various species, one primarily contributes to the charge transport, making the others referred to as "minority carriers". Given that anion mobility is influenced by mass, and all these distinct species originate in close proximity to the initial position of the primary charges, the discrepancy in the time of arrival of various anions effectively can be used as a means to measure the absolute position of the event along the z-axis. The third coordinate can be determined using the formula 
\begin{equation}
    z = \frac{v_m v_M}{v_m+v_M}\Delta t
\end{equation}
where $v_m$ represents the velocity of the minority carrier, $v_M$ is the velocity of the majority one, and $\Delta t$ is the arrival time difference between the two carriers.\\
\\
Within the CYGNO experiment framework, the objective of minimizing diffusion is to optimize the performance in determining directional parameters. Negative Ion Drift (NID) is considered as a potential method to achieve this goal. Given the significance of the charge gain and optical properties of He:CF4 for the detector's operation, a minimal amount of electronegative gas is introduced. The aim is to implement NID operation without altering the other gas characteristics. Hence, a 1.6\% concentration of SF$_6$ gas is introduced, aligning with measurements conducted in \cite{Baracchini_2018NID}, which confirmed NID operation with He:CF4. In this section, the results of negative ions drift operation with optical readout, obtained with the addition of a 1.6\% of SF$_6$ to the standard CYGNO gas mixture are reported.

\subsubsection{Anions mobility studies}
The detector employed for the NID operation studies in a CYGNO-like detector is the MANGO prototype. The drift gap was set to 5 cm, the maximum which can fit the gas-tight acrylic internal vessel, by employing a 5 cm field cage composed of 1 mm silver wires encased in 0.5 cm thick polycarbonate field rings with 7.4 cm internal diameter at 1 cm pitch. The field cage is enclosed on one side by a cathode made of a thin copper layer deposited on a PCB and on the other by the GEMs. A picture of the detector in this configuration with the alpha source installed is shown in \ref{fig:MANGOFcSmall}
\begin{figure}
    \centering
    \includegraphics[scale=.4]{figures/MANGOFcSmall.png}
    \caption{Picture of the MANGO detector with the 5 cm field cage setup. The disk on the side of the field cage is the alpha source employed.}
    \label{fig:MANGOFcSmall}
\end{figure}
To assess the drift velocity and mobility of the target gas mixtures, the PMT signal generated by alpha particles has been studied. An $^{241}$Am source was positioned at a 2.5 cm distance from the GEMs. Different measurements with various drift fields, specifically at 300 V/cm, 400 V/cm, 550 V/cm, and 700 V/cm have been conducted. In the Electron Drift (ED) configuration, the GEMs were operated at 310 V each, while in the Negative Ion Drift (NID) setup, GEM1, GEM2, and GEM3 were operated at 550 V, 545 V, and 540 V, respectively.\\ 
To measure the drift velocity the time extension of the PMT signal ($\Delta$T) has been used since the camera is not sensitive to this feature.
Through the measurement of $\Delta$T using the Electron Drift (ED) gas mixture, the corresponding $\Delta$z of the alpha can be determined given the knowledge of the drift velocity. Without relocating the source and by measuring $\Delta$T using the He:CF$_4$:SF$_6$ mixture with proportions of 59/39.4/1.6, it can be extrapolated the drift velocity for the Negative Ion Drift (NID) configuration, thanks to the prior knowledge of $\Delta$z. The plot of the drift velocity as a function of the drift field is shown in figure \ref{fig:NIDVelocity}. In the figure, it is also shown the results of an analysis performed in an identical way at the pressure of 650 mbar (Sec. \ref{sec:ImmAnalysis}) are also shown, together with the results published in \cite{Baracchini_2018NID} as a comparison.
Moreover, the reduced mobility ($v_{drift}/E$) of the ions as a function of the reduced field ($E/p$, where p is the pressure) is shown in the same figure.
\begin{figure}
    \centering
    \includegraphics[scale=.23]{figures/NidVelocity.png}
    \includegraphics[scale=.20]{figures/NIDReducedMob.png}
    \caption{Left: plot of the drift velocity as a function of the drift field applied for two different operating pressures, and the comparison with the work done in \cite{Baracchini_2018NID}. Right: plot of the reduced mobility calculated as a function of the reduced field for two different operating pressures, and the comparison with \cite{Baracchini_2018NID}.}
    \label{fig:NIDVelocity}
\end{figure}
The drift velocities measured at $\mathcal{O}$(cm/ms) clearly establish that the He:CF4:SF6 mixture at an operating pressure of 900 mbar enables Negative Ion Drift (NID). The results are consistent with the same analysis conducted using data collected at 650 mbar. The reduced mobility determined is comparable with the one presented in \cite{Baracchini_2018NID}. This last result have been obtained with a He:CF4:SF6 mixture at 360:240:10 Torr and was measured using pixel charge readout. The consistency among the three measurements is noteworthy, despite the high systematic uncertainties.

\subsubsection{Diffusion results from sCMOS picture analysis}
\label{sec:ImmAnalysis}
For this measurement, a different setup has been used. The detector was equipped with a 15 cm long field cage, manufactured exactly like the 5 cm one, and it was installed in a 150 l vacuum vessel made of stainless steel. In this configuration the light was collected with the same readout instrumentation, looking at the last GEMs through a quartz window featuring a 90\% transparency. The ORCA-Fusion camera is placed at a distance of approximately (26.6 $\pm$ 0.4) cm from the final GEM. In this setup, the camera captures an area measuring 14.1$\times$14.1 cm$^2$, resulting in an effective pixel size of 61$\times$61 $\mu$m$^2$.
Due to this setup, the solid angle was reduced by a factor of three, and to have a light output comparable to the one obtained with the previous setup, the operating pressure was reduced to 650 mbar.\\ 
In the case of Electron Drift (ED) operation, the GEMs are set at 310 V each. For Negative Ion Drift (NID) operation, GEM1, GEM2, and GEM3 are set at voltages of 535 V, 530 V, and 525 V, respectively. These GEM voltage settings are selected to achieve a similar light output for both gas mixtures in this configuration. For this study, the same $^{241}$Am source has been used and collimated with a paper window to avoid track spreading in z. To assess the diffusion of the gas mixtures used, data were collected at six different drift distances (2.5, 3.5, 4.5, 6.5, 9.5, and 12.5 cm from the GEMs) while varying the drift field strength (150, 200, 250, 300, 350, 400 and 600 V/cm) for both the Electron Drift (ED) and Negative Ion Drift (NID) gas mixtures at 650 mbar.\\ 
For the analysis, long and straight alpha tracks have been selected exploiting the track topology. The track has been cut in the central part to avoid border effect, and the transversal profile of the track has been fit with a Gaussian. From the mean value of the distributions of the $\sigma$ of the Gaussian, the diffusion parameter has been evaluated for each given configuration.
In figure \ref{fig:NIDDiff}, the measured diffusion is shown as a function of the drift distance for different drift fields applied. On the left side, the diffusion is shown for Electron Drift operations, while on the right, it is shown for Negative Ion Drift.
\begin{figure}
    \centering
    \includegraphics[scale=.4]{figures/NIDDiff.png}
    \caption{Diffusion measured for alpha tracks as a function of the distance for different values of drift field. The plots show the ED operations (right), and NID operations (left).}
    \label{fig:NIDDiff}
\end{figure}
The points have been fit with the function 
\begin{equation}
    \sigma_T = \sqrt{\sigma_0^2+\xi^2\cdot L}
    \label{eq:fitdiff}
\end{equation}
where $\sigma_T$ is the total diffusion measured, $\sigma_0$ represents the constant term of the diffusion happening in the GEM amplification plane, which does not depend on the drift distance, while $\xi$ represents the diffusion coefficient, thus how much the electron diffuse per unit of length, and L is the drift distance \cite{blum2008particle}. The results of the fit are reported in table \ref{tab:coeffValues}.
\begin{table}[h]
\centering
\begin{tabular}{|c|c|c|c|c|}
\hline Drift field $[\mathrm{V} / \mathrm{cm}]$ & $\sigma_0^{E D}[\mu \mathrm{m}]$ & $\xi^{E D}[\mu \mathrm{m} / \sqrt{\mathrm{cm}}]$ & $\sigma_0^{N I D}[\mu \mathrm{m}]$ & $\xi^{N I D}[\mu \mathrm{m} / \sqrt{\mathrm{cm}}]$ \\
\hline \hline 150 & $300 \pm 100$ & $280 \pm 20$ & $320 \pm 30$ & $110 \pm 10$ \\
200 & $290 \pm 60$ & $230 \pm 10$ & $260 \pm 30$ & $90 \pm 20$ \\
250 & $290 \pm 60$ & $210 \pm 10$ & $220 \pm 20$ & $81 \pm 10$ \\
300 & $300 \pm 40$ & $190 \pm 10$ & $220 \pm 20$ & $68 \pm 10$ \\
350 & $300 \pm 40$ & $170 \pm 10$ & $210 \pm 20$ & $60 \pm 10$ \\
400 & $310 \pm 30$ & $160 \pm 10$ & $210 \pm 20$ & $56 \pm 9$ \\
600 & $320 \pm 20$ & $140 \pm 10$ & $200 \pm 20$ & $45 \pm 10$ \\
\hline
\end{tabular}
\caption{In table the values of $\sigma_0$ and $\xi$ measured for electron drift and negative ions drift for the different drift field values are reported.}
\label{tab:coeffValues}
\end{table}
The values of $\sigma_0$ and $\xi$, coming from the results of the fits, as a function of the drift field applied for ED operations and NID. operations are reported in figure\ref{fig:NIDSigmaXiVsE}. 
\begin{figure}
    \centering
    \includegraphics[scale=.4]{figures/NidSigmaxiVsDF.png}
    \caption{Left: Plot of the $\sigma_0$ values as a function of the Drift field for the standard ED gas mixture and the NID gas mixture. Right: Plot of the $\xi$ diffusion parameter as a function of the drift field for ED and NID operation. The blue curve represents the thermal limit, while the higher and lower curves represent respectively the best fit with eq. \ref{eq:diffequation} for ED operation and NID operations. The pink points are the diffusion values obtained with the Garfield++ simulation.}
    \label{fig:NIDSigmaXiVsE}
\end{figure}
Additionally, the plot on the right shows respectively the expected thermal limit (blue curve) and the best fit result with eq. \ref{eq:diffequation} for ED operations (higher curve), and NID operations (lower curve). The pink points in the plot represent the result of electron drift diffusion from a Garfield++ simulation. As can be seen from the plot, the Garfield++ simulation fully matches the data for ED operation strongly validating the method and reinforcing the analysis results. For both of the gas mixtures, it is observed, as expected, a decreasing behavior with the increasing of the drift field value proportional to $1/\sqrt{E_{drift}}$. Nevertheless, while the ED curve shows a diffusion distinctly above the thermal limit, as expected for electrons, the NID data are characterized by a diffusion far below the thermal limit. 
From the eq. \ref{eq:diffequation} which relates the diffusion coefficient $\xi$ to the effective temperature $T_{eff}$ of the drifting charge carriers a temperature of 81 K can be derived for NID operation. This leads to a diffusion coefficient as low as 45 $\mu m /\sqrt{cm}$ at 600 V/cm which is a factor 3 smaller than the one measured in ED.
Another interesting feature, shown in the left panel of figure \ref{fig:NIDSigmaXiVsE}, is that the diffusion contribution from the GEM is lowered and diminishes with the increase of the electric field in the NID operations.

\subsubsection{Further Crosscheck}
To further confirm the analysis methodology, the experimental setup, and the presented results, the diffusion for the Electron Drift (ED) mixture is examined for different applied voltages on the GEMs. The objective of this cross-check is to illustrate that the analysis approach remains unaffected by the total light (and charge) produced in the GEM amplification plane, even at higher gains than the selected operating voltage for the discussed measurements thus far. This is crucial, since in case of gains too small a portion of the track, especially on the border, could end up below the detection threshold, affecting the sigma of the transverse profile. To demonstrate this, the drift field was set at 400 V/cm, while the voltage applied to each GEM varied from 290 V to 320 V (resulting in an overall voltage range from 870 V to 960 V). 
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{figures/DiffVsVGEM.png}
    \caption{Left: $\sigma$ of the transverse profile measured as a function of the distance from the GEM. Right: coefficient $\xi$ coming from the fit as a function of the GEM voltage.}
    \label{fig:VGEMVsDrift}
\end{figure}
The outcomes of this scan are presented in figure \ref{fig:VGEMVsDrift}, left plot, showing the sigma of the transverse profile as a function of the distance for different GEM voltages. The points have been fitted using equation \ref{eq:fitdiff}. The corresponding values of $\xi$ as a function of the GEM voltage are shown in the same figure, right plot. The data demonstrates no dependence of the measured diffusion on the GEM gain and thus on the light produced, increasing the robustness of the measurement.

\section{The future of CYGNO}
\label{sec:CYGNOFut}
The primary objective of the CYGNO project is to propel the development of gaseous Time Projection Chambers (TPCs) for the purpose of directional Dark Matter searches. Consequently, the future construction of a $\mathcal{O}(30) m^3$ detector for DM searches represents a significant point within the community of detectors with directional capabilities. To accomplish this aim, CYGNO is adopting a phased strategy that encompasses the creation of a 0.4 $m^3$ demonstrator, CYGNO-04, as an intermediate step towards the realization of the 30 $m^3$ experiment. In this section, these two forthcoming phases of CYGNO will be expounded upon.

\subsection{Phase\_1: CYGNO-04}
Drawing on the knowledge and insights gained from the construction, underground deployment, and operational phase of the LIME prototype, the CYGNO collaboration is advancing towards the establishment of a 0.4 $m^3$ experimental demonstrator for PHASE\_1, namely, CYGNO-04. The core objectives of PHASE\_1 encompass analyzing the employment of material with low radioactivity in the framework of a realistic experimental setup and scale, all while demonstrating the scalability and the strength of the detection technique towards a larger PHASE\_2 detector in terms of realizing the scientific objectives. The CYGNO-04 technical design report was presented to the LNGS administration and the pertinent funding agencies in July 2022. The CYGNO-04 installation is scheduled in Hall F in 2024. A scheme of the detector in Hall F with all the services needed in the experimental area is shown in figure \ref{fig:CYGNO04HallF}
\begin{figure}
    \centering
    \includegraphics[scale = .4]{figures/CYGNO04HallF.png}
    \caption{Scheme of the detector and the services adapted to the Hall F experimental area at LNGS}
    \label{fig:CYGNO04HallF}
\end{figure}
The detector will consist of two back-to-back TPCs with a common cathode, each of 50 cm drift length. Leveraging the experience acquired from the DRIFT collaboration, the cathode will consist of a 0.9 $\mu m$ aluminized Mylar foil \cite{Daw:2011wq,Battat_2015}. The use of aluminum coating is advantageous as it does not introduce radioactive materials. Moreover, the film's thickness permits alpha particles originating from radon daughter decays to release energy in the fiducial volume, facilitating event tagging and elimination. In order to further mitigate internal background interference, the field cage will be fabricated from a single Kapton foil, with thin copper layers printed on it that operate as rings. This method, previously used by the DRIFT collaboration, eliminates the need for ceramic resistors typically found in conventional field cages which are highly radioactive. Simultaneously, it minimizes the copper content and thus the presence of radioactive materials. The amplification stage encompasses a 50 × 80 cm$^2$ area and will be featured by three 50 $\mu$m thin GEMs. To further mitigate the radioactive contamination of this component, a cleaning technique based on DI water baths, as developed by the T-REX collaboration, will be employed \cite{Castel_2019}.
The detector will be enclosed in a PMMA acrylic vessel for the purpose of reducing material radioactivity, preventing gas contamination, and ensuring electrical insulation from the internal electrodes.
The optical readout configuration includes six PMTs and two sCMOS cameras on each side to cover the entire amplification area. The selected PMT model is the Hamamatsu R7378A, which offers a 15\% quantum efficiency, particularly at long wavelengths, such as 550 nm \cite{Antochi_2018}. Given the usual low radioactivity of PMTs and their positioning at a significant distance, their contribution to the background levels can be considered negligible. As sCMOS cameras, the Hamamatsu ORCA QUEST will be used. This innovative sensor exhibits enhanced noise performance in comparison to the ORCA Fusion (Sec. \ref{sec:camera}), with approximately 0.27 electrons RMS. This allows each pixel to perform single-photon counting while maintaining an effective granularity of approximately 200$\times$200 $\mu$m per pixel in the CYGNO-04 configuration. Due to the significant $^{40}$K contamination observed in the camera lens, the CYGNO-04 project is currently collaborating with external companies to develop customized lenses made from ultra-pure silica (SUPRASIL). This initiative is expected to lead to the production of lenses with radioactive contamination from these components by approximately a factor of 10$^4$ less. Additionally, the collaboration is working to minimize the radioactive contribution from the sCMOS camera. This involves customizing the readout electronics to place them outside the shielding and replacing the sCMOS sensor protective glass window with one made of ultra-pure silica.
A detailed scheme of the detector with all the components is shown in figure \ref{fig:cygno04scheme}.
\begin{figure}
    \centering
    \includegraphics[scale=.4]{figures/CYGNO_04_scheme.png}
    \caption{In figure the schematic representation of the CYGNO-04 detector illustrating all its components is shown.}
    \label{fig:cygno04scheme}
\end{figure}
A preliminary GEANT4 simulation was conducted to assess the expected radioactive background in CYGNO-04, considering both external and internal material radioactivity. The purpose of this simulation was to refine the selection of the materials to use as shielding. The preliminary choice for the shield, which also considers the constraints of available space in Hall F, consists of a 10 cm layer of copper enclosed in 1.1 meters of water. This configuration is found to reduce the external radioactive contribution to the background to the level of approximately 1/20 of the internal one.
Due to the modular design of CYGNO-04 and the insights gained from the fiducial cuts from the background studies (Sec. \ref{sec:bkgStudies}), a comparable potential for background reduction is foreseen with volume fiducialization. In addition to this, initial investigations into gamma background rejection using a Deep Neural Network algorithm, which relies on track shape variables extracted from sCMOS images, indicate a remarkable 98.3\% rejection along the entire [1-40] keV$_{ee}$ range, while maintaining a 40\% nuclear recoil efficiency. The continuous improvement in sCMOS camera sensitivity, coupled with the integration of PMT data, holds the potential to substantially enhance these initial performances. Additionally, the implementation of Convolutional Neural Networks that combine sCMOS and PMT information promises to further refine the results. Therefore, one can anticipate an expected background level of approximately 10-100 events per year in the 1-20 keV$_{ee}$ region for CYGNO-04. The CYGNO-04 Technical Design Report was submitted in July 2022 and has received approval from LNGS management and the funding agency.

\subsection{Phase\_2: CYGNO-30}

A CYGNO-30 experiment has the potential to make a substantial contribution to the Dark Matter searches in the range of masses below 10 GeV, encompassing both Spin-Independent (SI) and Spin-Dependent (SD) coupling interactions. In case of other experiments would claim a DM observation, CYGNO's directional capabilities would play a decisive role in definitively confirming the Galactic origin of an eventual DM signal. Moreover, with such a detector it would be possible to study the DM halo substructure \cite{MAYET20161}. \\
Apart from its contribution to Dark Matter (DM) research, such an experiment can also have relevance in the field of neutrino physics.
CYGNO-30 could open the way for a directional measurement of solar neutrinos from the pp chain via elastic scattering on electrons, potentially expanding the energy range of the Borexino findings \cite{borexino2018comprehensive} down to $\mathcal{O}(10)$ keV. Traditional dark matter experiments, which lack directional sensitivity in their event detection, are unable to differentiate between electron recoils induced by solar neutrinos and those arising from natural radioactivity \cite{instruments6010006}. In contrast, a directional detector such as CYGNO can exploit the directional information to discriminate electron recoils resulting from solar neutrino interactions. These interactions exhibit a highly peaked asymmetric angular distribution, over the flat angular distribution of electron recoils coming from background sources. Coincidentally, the CYGNO mixture contains CF$_4$ gas, which possesses a high electron density (approximately 10$^{21}$ cm$^{-3}$) relative to its low average atomic number (Z). This characteristic mitigates the issue of multiple scattering of low-energy electron recoils within the gas. The reduction of multiple scattering is particularly significant since it facilitates the determination of the initial direction for low-energy electron recoils.\\
Another physics case for CYGNO-30 could be physics beyond the standard model in Coherent Elastic Neutrino-Nucleus Scattering (CE$\nu$NS) interactions.
The Coherent Elastic Neutrino-Nucleus Scattering serves as the fundamental process responsible for the "neutrino fog" below which the Dark Matter signal starts to be indistinguishable from a neutrino one. Although a detector with an $\mathcal{O}(30) m^3$ volume may not provide sufficient exposure to detect Solar neutrino events through CE$\nu$NS interaction, the presence of new physics phenomena in the neutrino sector could potentially enhance the CE$\nu$NS cross-section at low energies, resulting in a considerable increase in event rates by several orders of magnitude\cite{B_hm_2019,Bertuzzo_2017}.\\
A sketch of a possible configuration of a 30 $m^3$ CYGNO Phase\_2 detector assembled in Hall C of the underground laboratories at LNGS is shown in figure \ref{fig:CYGNO30}.
\begin{figure}
    \centering
    \includegraphics[scale=.35]{figures/CYGNO30.png}
    \caption{Sketch of a 30 $m^3$ CYGNO Phase\_2 detector in Hall C at LNGS. }
    \label{fig:CYGNO30}
\end{figure}
Given the modularity of the CYGNO approach, a CYGNO-30 detector could be, in a first concept, composed of 75 CYGNO-04 modules. These modules will be arranged in three vertically stacked rows, and each row will be composed of 25 modules. A conceptual design of the CYGNO-30 detector will be presented in Sec. \ref{chap:solarnu}, in the context of the background studies for the sensitivity to the directional solar neutrino measurement. 

\subsubsection{R\&D lines for CYGNO Phase\_2}
One potential approach to enhance sensitivity in the low WIMP mass region while maintaining the same energy threshold is to include very light elements in the gas mixture, for a more efficient momentum transfer at lower WIMP masses. Hence, the collaboration is exploring the feasibility of introducing hydrogen-rich molecules into the CYGNO gas mixture. This can be achieved by adding a small proportion of either iC$_{4}$H$_{10}$ or CH$_{4}$. It has been observed that both gases modestly reduce the photon-to-electron ratio production. However, when methane is used, the amplification system exhibits greater stability, and the GEM voltages can be increased by around 70 V. This voltage increment can yield a higher light yield without compromising the detector's stability.\\
Achieving significant amplification in the optical readout is crucial due to the limited coverage of these sensors over a small solid angle. An enhancement in light production is essential for improved sensitivity to lower WIMP masses. In this context, the potentiality of introducing a high electric field after the outermost GEM to enhance photon production in the high field region under electroluminescence is under investigation.

==> chapters/XRayAnalysis.tex <==

\chapter{Analysis of LIME response to low energy electron recoils}
\label{ch:XRayAn}
In order to evaluate CYGNO experimental approach capability to detect low energy electron recoils, LIME was exposed to X-rays with energies from 3.5 keV to 35 keV, and its response to them was thoroughly analyzed. In this Chapter, we will illustrate the experimental setup and dataset acquired (Sec. \ref{sec:setupXray}), the reconstruction algorithm employed to analyze the data (Sec. \ref{chap:reco}), and the energy response linearity and resolution evaluated from this data (Sec. \ref{sec:analysis}).

\section{Experimental Setup}
\label{sec:setupXray}
In this section, a comprehensive overview of the detector's operational conditions will be provided, together with a detailed description of all experimental apparatus, and insights on the radioactive calibration sources employed.


\subsection{Detector operative conditions}
The data taking has been conducted with our largest prototype, LIME, described in detail in Sec \ref{sec:LIME}. It was filled with a gas mixture of He:CF$_4$  (60:40), and it was operated with a constant flux of 9 L/h, for the whole data taking. The detector was configured to its standard operational settings $V_{G1}=V_{G2}=V_{G3}=440$V, $V_{tr1}$ = $V_{tr2}$ =2.5 kV/cm and $V_{drift}=940$ V/cm. For the cooling of the camera, the water cooling system was employed, using water at 25° During the operation the camera was operated in free running mode and the images were acquired with the Hamamatsu Hokawo software. The data taking was performed overground and without shield from external radiation. For this reason, an acquisition time of 50 ms was chosen to handle the high occupancy of cosmics and high energy electrons from natural radioactivity in the images. The difference between a sCMOS image acquired with 300ms and 50ms exposure is shown in figure \ref{fig:expdiff}.

\begin{figure}
    \centering
    \includegraphics[scale=.4]{figures/300msOcc.png}
    \includegraphics[scale=.28]{figures/50msOcc.png}
    \caption{Pictures acquired with the sCMOS with 300/50ms exposure left/right }
    \label{fig:expdiff}
\end{figure}

Prior to data acquisition, the GEMs were turned off, and a set of 400 pictures at the same exposure was acquired in order to measure the camera's baseline, commonly referred to as "pedestal". The pedestal will be later subtracted at reconstruction level from the sCMOS picture acquired. 
The signal in the detector was induced in the detector by means of X-rays at different energies. For the X-ray production, two different radioactive sources were employed. The sources and the methods used for the X-ray production are described in detail in Sec. \ref{sec:multisource}. For each energy, a set of 4000 pictures has been acquired.

\subsection{Multi-energy X-Ray production}
\label{sec:multisource}
In this section, a detailed description of the radioactive calibration sources utilized will be provided. Specifically, the $^{55}Fe$ source and the $^{241}$Am source will be described, together with the methodologies employed to generate monochromatic X-rays at various energies starting from these two sources.

\subsubsection{The Amersham multi-energy X-Ray source}
One of the multi-energy X-ray sources employed is the Amersham AMC.2084. This consists of a 370 MBq $^{241}$Am source producing $\sim$5 MeV alpha particles, directed onto disks composed of different materials placed on a rotating support. The materials used are copper (Cu), rubidium (Rb), molybdenum (Mo), silver (Ag), barium (Ba), and terbium (Tb), and they can be selected through the rotation of a wheel. The wheel rotation causes the disk to be in correspondence with an aperture for the passage on the X-Ray. A scheme of the source is reported in figure \ref{fig:source1}.

\begin{figure}
    \centering
    \includegraphics[scale=.3]{figures/AMC2084.png}
    \caption{Scheme of the Amersham AMC.2084 variable energy X-ray source}
    \label{fig:source1}
\end{figure}

Upon interaction with the materials, the alpha particles, through ionization, cause the ejection of an electron from the atom's inner shell, K-shell. An outer-shell electron, from the M-shell or L-shell, filling the vacancy causes the production of a monochromatic X-ray, resulting in what is respectively named $k_{\alpha}$ and $k_{\beta}$ emissions. A schematic view of the process is shown in figure \ref{fig:CharRad}. 

\begin{figure}
    \centering
    \includegraphics[scale=.14]{figures/kemission.png}  
    \caption{In figure the scheme of X-ray production for different electronic transitions after an external stimulation is shown.}
    \label{fig:CharRad}
\end{figure}

The energy of the emitted gamma will be equal to $ E_{\gamma}=E_{K-shell}-E_{M/L-shell}$, where $E_{X-shell}$ represents the bounding energy of the electron in the X-shell. Given that $\Delta E_{M-L}<<\Delta E_{K-ML}$, the resulting emission spectrum will consist of two closely spaced lines, each centered at the respective $E_{\gamma}$. 
The spectrum resulting from the emission of the materials described above is shown in figure \ref{fig:gamma_emission_E}, and the energies of the photons for both $k_{\alpha}$ and $k_{\beta}$ emissions are reported in table \ref{tab:gamma_emission_E}. As can be seen from the plot the yield for the $k_{\beta}$ emission is $\sim$20\% of the $k_{\alpha}$. This happens because the selection rules for electronic transition favor the $k_{\alpha}$ emission.

  \begin{minipage}{\textwidth}
  \begin{minipage}[!t]{0.45\textwidth}
    \centering
\includegraphics[scale=.5]{figures/SourceSpectrum.png}  
    \captionof{figure}{In the figure the spectrum of the source is shown for all the target materials}
    \label{fig:gamma_emission_E}
  \end{minipage}
  \hfill
  \begin{minipage}[!t]{0.45\textwidth}
    \centering
    \begin{tabular}[]{|c|c|c|}                          
    \hline                                                     
        Element & $k_{\alpha}$ \ [keV] & $k_{\beta}$ \ [keV] \\ \hline   Cu & 8.04 & 8.91 \\ \hline                                       
        Rb & 13.37 & 14.97 \\ \hline                                     
        Mo & 17.44 & 19.63 \\ \hline                                     
        Ag & 22.10 & 24.99 \\ \hline                                     
        Ba & 32.06 & 36.55 \\ \hline                                     
        Tb & 44.23 & 50.65 \\ \hline                                     
    \end{tabular}
      \captionof{table}{In the table the energy of the photons for the different $k_{\alpha}$ and $k_{\beta}$ emissions are \
reported}
    \label{tab:gamma_emission_E}
    \end{minipage}
  \end{minipage}

The gammas interact in the detector through the photoelectric effect and will produce electron recoils. Pictures of the ER resulting from X-ray interaction at different energies are shown in figure \ref{fig:multiEtracks}.

\begin{figure}
    \centering
    \includegraphics[scale=.45]{figures/MultiTracks.png}
    \caption{In figure the electron recoils produced by gammas at different energy }
    \label{fig:multiEtracks}
\end{figure}
 It can be observed that the tracks appear like a spot at the energy of 8 keV. This occurs because at that energy the distance covered by the electron traveling in the gas is considerably smaller than the size of the diffused tracks. The tracks start to exhibit a significant extension for energies above 15 keV. The source was positioned at the upper section of the detector in correspondence of the thin EFTE window, at the middle point of the sensitive volume along the drift direction.

\subsubsection{The $^{55}$Fe source and, Ti and Ca X-ray stimulated emission}

To investigate the detector's response at energies below 8 keV a 740 MBq source of $^{55}$Fe has been employed. The $^{55}$Fe undergoes electronic capture with 100\% probability, resulting in the production of a $^{55}$Mn atom lacking an electron in the K-shell. Subsequently, this atomic configuration will further produce a $k_{\alpha}$ or $k_{\beta}$ emission emitting an X-ray of 5.9 keV or 6.5 keV, respectively with a $\sim$ 13\% probability associated with the occurrence of a $k_{\beta}$ emission. 

For the production of further lower energy X-ray, the same $^{55}$Fe source has been used to irradiate with gammas a titanium (Ti) sheet and chalk pieces containing Calcium (Ca). These elements have an energy for the $k_{\alpha}$ emission of 4.5 keV and 3.7 keV, respectively. The setup in these configurations is shown in figure \ref{fig:CaTiSource} where the collimator for the X-ray from the target material to the detector is also shown.

\begin{figure}
    \centering
    \includegraphics[scale=.3]{figures/TiSource.png}
    \includegraphics[scale=.5]{figures/CaSource.png}
    \caption{The pictures show the experimental configurations used for the production of 4.5 e 3.7 keV X-ray from titanium and Calcium.}
    \label{fig:CaTiSource}
\end{figure} 



\section{The track reconstruction code}
\label{chap:reco}
As can be seen in figure \ref{fig:multiEtracks} particle interactions in the detector result in light clusters captured in the sCMOS picture. To reconstruct these tracks, a dedicated dynamic algorithm has been developed by the CYGNO collaboration. The algorithm is designed for efficient reconstruction of the tracks released by different kind of particles, each showing distinct energy release patterns and geometric characteristics. It is indeed able to recognize very low energy nuclear recoils consisting of tiny dense light spots, long and straight tracks induced by cosmic rays crossing the detector volume, or curly with non-constant energy ionization profiles tracks generated by electrons crossing the sensitive volume. The reconstruction algorithm needs therefore to efficiently be able to reconstruct all these different patterns. 
For these reasons, the analysis of the sCMOS images proceeds through four steps, by firstly dealing with the intrinsic noise sensor (Sec. \ref{sec:prelim}) and the optical distortion of the system (Sec. \ref{sec:vignetting}), and subsequently finding basic clusters from the single small deposit (sec \ref{sec:dbscan}), which are eventually merged into the full tracks that represent the output of the reconstruction (Sec. \ref{sec:finaldbscan}).
The output generated by the reconstruction code comprises a set of x-y coordinates of the pixel constituting each track along with their respective intensities. The sum of the pixel intensity provides a quantity proportional to the energy of the track. Moreover, from the single pixels information important topological quantities can be derived. These include, among others, the specific ionization along the track $dE/dl$, or the total light density $\delta=E/npixels$. This is a distinctive aspect of this kind of detector, which allows for the track direction and sense recognition, and particle discrimination by leveraging these topological track variables.

\subsection{Sensor noise reduction}
\label{sec:prelim}

A sCMOS picture acquired by the camera consists of an array of 2304x2304 pixels with intensity expressed in ADC counts. The amplification process of photoelectron conversion to an electric signal, the heat-generated ionization in the silicon sensor, and the electrical connections are all sources of noise \cite{Lundberg2002NoiseSI}. 
To handle this noise, the set of images taken with GEMs turned off is used. In the absence of any source of light, the images acquired with the camera contain only counts related to the pixel noise. Consequently, from those images, it is possible to perform a statistical analysis to characterize the mean value and the RMS of the noise present in each pixel. By calculating the average and the RMS of the pixel intensity, it is obtained an average value of $\sim$ 100 counts and a standard deviation of $\sim$ 3.7 counts. The distributions of the mean values and RMS values of the pixels calculated averaging on 400 pedestal images acquired for the multi-energy X-ray data acquisition campaign are shown in figure \ref{fig:PixelsMeanRMS}. The tails present on the right sides of the distributions are due to the pixels located at the top and bottom borders of the sensor, which were particularly noisy in the camera used for this analysis. 
\begin{figure}
    \centering
    \includegraphics[scale=.38]{figures/MeanPed.png}
    \includegraphics[scale=.38]{figures/RMSPed.png}
    \caption{Left/right: distribution of the pixels mean/RMS values for the 400 pedestal images acquired for the multi-energy X-ray data acquisition campaign}
    \label{fig:PixelsMeanRMS}
\end{figure}
From this information, a pedestal map is built. This map consists of two separate 2304x2304 matrices containing the information of mean $\bar{N}_{i,j}$ and RMS $\sigma_{N i,j}$ of each pixel $i,j$. 

In order to reduce the noise, the pedestal map is subtracted pixel by pixel to each sCMOS image. Subsequently, to further reduce the noise, a zero suppression operation has been performed on the pedestal subtracted image. By defining $C_{ij}$ the content of each pixel after the pedestal subtraction, the condition for the pixel to survive the zero suppression is 
\begin{equation}
    C_{i,j}> n_\sigma \cdot \sigma_{Nij}
\end{equation}
where $n_\sigma$ is a parameter of the algorithm that is optimized before the reconstruction process depending on the noise condition of the dataset. In this case, the parameter $n_\sigma$ was just set above the noise level, specifically to $n\sigma$=1.2. This choice was made to ensure good detection efficiency while preventing overloading of the reconstruction algorithm with pixels dominated by noise.
Images are subsequently rebinned (4x4) for CPU reasons into images of 576x576 macro-pixel. The charge of each macro-pixel is calculated as the average of the charge from the 4x4 pixels composing it. 
The rebinned image is then processed using a 3x3 median filter, a local image filtering technique commonly used for noise reduction purposes. For each pixel of the image, a square of 3x3 pixels (called kernel) around the designed one is considered. The value of the designed pixel is then substituted in a new image with the median value of all the pixels in the 3x3 square \cite{Welk_2016}.
The working scheme of the median filter is illustrated in figure \ref{fig:medianfilter}.
\begin{figure}
    \centering
    \includegraphics[scale=.5]{figures/medianfilter.png}
    \caption{In the picture the working mechanism of the median filter is shown. The central pixel of value 200 is replaced by the median value of all the pixels in a 3x3 square around the central one, in this case, 94.}
    \label{fig:medianfilter}
\end{figure}

\subsection{Vignetting correction}
\label{sec:vignetting}
The resulting image is then corrected for the vignetting effect caused by the camera lenses.
In an optical system like the one used in CYGNO, in which an objective with two lenses is employed, it occurs that the first lens can direct the light in a way that only a fraction of it reaches the second lens, and is directed towards the sensor. The images, thus, appear progressively darker going far from the center of the picture, when capturing a uniformly illuminated scene.
The working scheme of this effect is shown in figure \ref{fig:vignettingphen}, where the different behavior of light from an on-axis and an off-axis point is shown \cite{Goossens_2019}. As can be seen, the darkening is more pronounced for part of the object off-axis with respect to the center of the sensor.

\begin{figure}
    \centering
    \includegraphics[scale=.4]{figures/VignPhen.png}
    \caption{The picture describes the vignetting effect. The light coming from the points of an object off-axis is partially cut by the camera lens.}
    \label{fig:vignettingphen}
\end{figure}

More in detail, the intensity $I$ of the light due to this effect is maximal when the object is on-axis $\phi$=0 and decreases proportionally to $I\propto cos(\phi)^4$, where $phi$ is the angle that the object form with respect to the lens axis \cite{10.1088/978-0-7503-2558-5}.

In order to properly correct for this effect on the acquired images, the vignetting has been characterized by exposing the camera to a white wall illuminated with light to simulate a "uniformly illuminated" setup).  Different pictures of the wall have been acquired with the camera in a horizontal position and rotated with steps of $90°$. Subsequently, a vignetting map has been constructed by averaging the light intensity in the pictures and normalizing it to the maximum value of the ADC counts. 
The vignetting correction is then applied to the sCMOS data images by multiplying each pixel $i,j$ by the value $1/V_{i,j}$, where $V(i,j)$ is the value of the vignetting map in the pixel $i,j$.

\subsection{The iDBSCAN algorithm}
\label{sec:dbscan}
Once the preliminary operations are concluded, the official CYGNO reconstruction \cite{Baracchini:2020nut} code based on the Density-Based Spatial Clustering of Applications with Noise (DBSCAN) \cite{scikit-learn} algorithm is used to identify and reconstruct the light clusters. 
DBSCAN is capable of clustering high-density areas separated by low-density areas within a picture. The clustering operation relies on both the distance between pixels and their intensity as rules for cluster formation. 
These operations are performed driven by two parameters: $\epsilon$ and $N_{min}$. Whenever the number of points within a radius $\epsilon$ centered in a selected point (randomly chosen seed) is greater than $N_{min}$, the clustering process starts. The seed point is marked as part of the cluster, and the sampling procedure proceeds by iterating through every point found within $\epsilon$ in the previous iteration. A point is labeled as a core point if it has $N_{min}$ neighbor within a radius $\epsilon$, if this condition is not satisfied, a point is marked as a border-point. Any points not satisfy the condition of core-point or border-point are marked as noise. The cluster is finally formed by the union of core points and border points \cite{scikit-learn}. A scheme of the DBSCAN working principle is shown in figure \ref{fig:DBSCAN}.
\begin{figure}
    \centering
    \includegraphics[scale=.6]{figures/DBSCANproc.png}
    \caption{In figure the DBSCAN working principle is shown. The black points having at least 4 points within a radius $\epsilon$ are marked as core points. The blue points are found close to a core point but do not satisfy the requirement of the minimum number of points, so they are marked as border points. The red points are noise.}
    \label{fig:DBSCAN}
\end{figure}
In CYGNO, alongside the information on the coordinate of a point, the intensity information is also used. Therefore an intensity-based version of the DBSCAN (iDBSCAN) algorithm is used.
In iDBSCAN the condition of the minimum number of points $N_{min}$ to form a cluster is substituted with the requirement of a minimum intensity among neighbor points. As demonstrated in \cite{Baracchini_2020}, the iDBSCAN algorithm, on CYGNO images, shows an improved background rejection efficiency compared to both the standard DBSCAN and a Nearest Neighbor Clustering method.

\subsection{Cluster formation}
\label{sec:finaldbscan}
To handle the high pileup generated by cosmics and high energy electrons, a dedicated algorithm based on iDBSCAN is used to reconstruct and remove this source of background. These types of tracks can be approximated by linear and high-degree polynomial curves. As a result, the directional information of the cluster is employed to enhance the algorithm ability in the identification of this background source.
A key component of this directional iDBSCAN (iDDBSCAN) is the RANdom SAmple Consensus (RANSAC) algorithm. RANSAC is an iterative method used to determine the optimal parameters of a model in a set of data containing a large proportion of outliers. This is realized by (1) selecting a random subset of data of size $m$ from the overall dataset of size $M$, (2) fitting the selected data with the model, and (3) evaluating the number $i$ of inliers points which are within a distance $\omega$ from the fitted model. The sequence of steps 1 to 3 can be iterated $N$ times. The model with the highest number of $i$ is the most suitable one for accurately representing the data omitting the effect of the outliers \cite{RANSAC}. The difference between a linear fit and a RANSAC regression is shown in figure \ref{fig:RANSAC}. 
\begin{figure}
    \centering
    \includegraphics[scale=.6]{figures/RANSAC.png}
    \caption{Comparison of a linear and a RANSAC regression. The outlier points influence the goodness of the linear regression, while RANSAC shows robust fitting on the inliers.}
    \label{fig:RANSAC}
\end{figure}
\\
It can be estimated that given $w$ as the actual fraction of inliers, $p$ the desired probability of finding a subset of data without outliers, the average number of iterations $k$ required for this condition is:  
\begin{equation}
    k= \frac{log(1-p)}{log(1-w^n)}
\end{equation}
with $n<w \cdot M$. To provide an idea, given a model with $w=0.8$, by choosing $n=10$ and $p=0.9$ the resulting number of iterations is $k=20$. 


In light of this, the algorithm performs a first seeding, applying an iDBSCAN iteration to the whole image. After this procedure, each identified cluster with coordinates ($x_i,y_i$) is tested with a linear-RANSAC ($y(x)$). The parameters used are $m=1/2\cdot M$ (50\% pixels), and $\omega$=1 MAD (Median Absolute Deviation), where 1 MAD is defined as 
\begin{equation}
    1 MAD = median(|y_i-median(y_i)|)
\end{equation} %ricomincia da qui
The procedure is terminated and the cluster is marked as directional the inline ratio reaches $i/M>0.8$. If no directional cluster is found the algorithm execution is concluded, and the result is given by the iDBSCAN clustering. 
If a directional match is found the algorithm proceeds with the directional clustering. For a cluster marked as directional, the iDBSCAN procedure is applied. Subsequently, a third-order polynomial RANSAC is executed. iDBSCAN is then executed in a region of size $\omega$ centered around the optimal third-order polynomial model found for the cluster. For the directional searches a radius $\epsilon_{dir}$ different from $\epsilon$ is used. The procedure continues until no more pixels can be added to the cluster. Once the procedure is ended it is repeated for any other directional cluster and continues until all directional clusters are processed. 
After this procedure, an additional step for noise reduction is performed. Any pixels with a certain distance $\rho_{isolation}$ from a directional cluster reconstructed are marked as noise, and are excluded in the final step. This is to prevent additional cluster formation close to cosmics and high-energy electrons. Since these tracks are very long, the probability of finding noise around that can become part of the cluster is not negligible. 
Finally, iDBSCAN is applied to all the pixels not included in a directional cluster and not marked as noise. After an exhaustive parameter optimization and validation, described in detail in \cite{Amaro_2023}, the X-ray runs reconstruction has been performed. 
In figure \ref{fig:picReco}, from left to right, are shown: the original image, the tracks reconstructed with iDBSCAN, and the tracks reconstructed with iDDBSCAN are shown for an event in the Rb dataset. Pixels with the same color belong to a single track.
\begin{figure}
    \centering
    \includegraphics[scale=.19]{figures/RbOri.png}
    \includegraphics[scale=.19]{figures/RbSeeding.png}
    \includegraphics[scale=.19]{figures/RbDirSearch.png}
    \caption{Left:Original picture from sCMOS camera, center: iDBSCAN seeding, right: iDDBSCAN clustering }
    \label{fig:picReco}
\end{figure}
The pixels x-y position, and the number of counts of each pixel associated with each track are then used to analyze the data.

\section{Analysis of X-Ray data}
\label{sec:X-RayAnalisys}
The sum of the counts associated with a track, thus the light integral, is proportional to its energy.
The data analysis for detector response, and track shape variables, has been based on an unbinned likelihood fit. For the model, the background is expected to have an exponential shape, whereas the signal is expected to follow a Gaussian distribution. From the result of the fit, the response of light counts as a function of the energy has been studied as well as the energy resolution. Furthermore, with the $sPlot$ tool the topological variables of the tracks for pure signal and pure background have been extracted for a subsequent topological variables comparison with the Monte Carlo simulation. 

\subsection{The fit models and data selection}
The distribution of light integral from the monochromatic X-ray data has been fitted with two exponential to model the background, and Gaussians to model the signals.
A part of the background, as shown in \cite{Costa_2019}, is composed of fake clusters, with falling exponential energy distribution. The second exponential function is used instead to model the real physics background, originating from electrons and cosmics interacting in the detector.
To model the signal, depending on the case 1 or 2 Gaussian are used. X-rays with energies higher than 8 keV are capable of extracting additional electrons from the copper comprising the field cage bars. For this reason, the signal coming from these sources is expected to be composed of two components, one centered at the x-ray energy and a second one at 8 keV, which is the x-ray emission line from Cu. 
For the $^{55}$Fe, given the high intensity of the source, there was a non-negligible probability of having two very close iron spots in space. In such an instance, the reconstruction algorithm, merging the close spots, gives rise to a second peak at an energy double the iron one. 
For Ti, even if the source was shielded a large amount of residual $^{55}$Fe was present in the pictures. In the analysis phase, the Ti Gaussian peak was observed to be completely covered by the iron one, leading to a non-trustable result. The data from Ti will not be considered in this thesis.

For each dataset, a very loose data selection has been made as follows:
\begin{itemize}
\setlength\itemsep{0em} 
    \item  light integral $>$ 100 to remove the noise
    \item  track length $<$ 400 to remove very long tracks
    \item  track barycenter within 800 pixels from the center of the picture
    \item  pixel light RMS $>$ 6 to further remove noise
\end{itemize}

Considering the very low attenuation length of gammas from Ca, the majority of the interactions in the detector occurred very close to the top border of the detector. Therefore, a different geometrical selection has been applied $900<x<1400$ and $2000<y<2200$.


\subsection{Unbinned maximum likelihood fit}
\label{sec:likelihood}
The technique used to perform the fit of the energy spectrum is the unbinned maximum likelihood fit. This technique indeed is more robust than the binned method when a small number of events is present and allows for the statistical subtraction of the background contribution via the $_{s}\mathcal{P}\textrtaill{lot}$ formalism as described in section \ref{sec:splot} and in more detail in appendix \ref{app:appendixA}.
Considering a random variable x characterized by a probability density function (p.d.f.) $f(x|\Vec{\theta}\ )$, with $f$ known but any or part of the parameters of the function $\Vec{\theta}=(\theta_1,\theta_2,...,\theta_n)$ unknown, the maximum likelihood method can be used to obtain the best estimation of $\Vec{\theta}$ $\rightarrow$ $\Vec{\theta}_{best}$ from the data. The resulting p.d.f. $f(x|\Vec{\theta}_{best}\ )$ is the one which effectively describe the data distribution. 
%Given a set of event $\Vec{x}=(x_1,..,x_n)$ described from the p.d.f. $f(\Vec{x}|\Vec{\theta}\ )$, the probability for the fist event to be in $[x_1,x_1+dx_1]$ will be $f(x_1|\Vec{\theta}\ )dx_1$. A second event will have a probability of being in $[x_2,x_2+dx_2]$ equal to $f(x_2|\Vec{\theta}\ )dx_2$. 
For a set of N events, the joint probability of each $x_i$ to be within $[x_i,x_i+dx_i]$ will be equal to
\begin{equation}
    p(x_i \in [x_i,x_i+dx_i] \ \forall i) = \prod_{i=0}^{N}{f(x_i,\Vec{\theta}\ )dx_i}
\end{equation}

If the hypothesis on $f$ and the values of $\Vec{\theta}$ are correct in describing the data, it is expected a high probability for the data measured. In the opposite case, the probability will be low. On the basis of this, it can be defined a likelihood function, which represents the likelihood of a given set of data to be described by the p.d.f. with given parameters:
\begin{equation}
    \mathcal{L}(\Vec{\theta}\ ) = \prod_{i=0}^{N}{f(x_i,\Vec{\theta\ })}
\end{equation}
Once the experiment is done, the set of $\Vec{x}$, being the data acquired, are fixed numbers, thus $\mathcal{L}$ is only a function of the parameters $\Vec{\theta}$. Maximizing the likelihood on the data with respect to $\Vec{\theta}$ gives the best estimate for the parameters
\cite{Cowan:1998ji}. From an operative point of view, the -$log(\mathcal{L})$ is considered. This is because the values that $\mathcal{L}$ can assume span many orders of magnitude, and it is easier to work with sums than with products ($log(ab)=log(a)+log(b)$). Thus it will be more efficient and more stable for a calculator to minimize this quantity.

In case of a single Gaussian signal ($s$) with mean $\mu$ and standard deviation $\sigma$, and 2 exponential backgrounds ($b_1$,$b_2$) with parameters $\alpha_1$ and $\alpha_2$, the respective p.d.f. for $s$ and $b$, namely $f_s$ and $f_b$ can be written as
\begin{align}
 &f_s(x_i| \mu,\sigma)=\frac{1}{\sqrt{2\pi\sigma^2}}e^{-\frac{1}{2}\left(\frac{x_i-\mu}{\sigma}\right)^2} \\  
 &f_{b}(x_i| \alpha_1,\alpha_2,c) = c\cdot \frac{1}{\alpha_1}e^{-\frac{x_i}{\alpha_1}}+(1-c)\cdot \frac{1}{\alpha_2}e^{-\frac{x_i}{\alpha_2}} \ \ with \ \  0<c<1
\end{align}

Here, the parameter $c$ takes into account the probability for an event to belong to the first type of background or the second. Using the expression $f_{b}=c \cdot f_{b1}(x_i,\alpha_1) + (1-c) \cdot f_{b2}(x_i,\alpha_2)$ guarantees the normalization of $f_b$ and allows to use an overall $N_b$ parameter for the total number of background event.
Defining $N_s$ and $N_b$ respectively the number of events for $s$ and $b$, and $\Vec{\theta}=(N_b,N_s,\mu,\sigma,\alpha_1,\alpha_2,c)$, the p.d.f. which describes the total distribution, can be written as
\begin{equation}
    f(x_i,\Vec{\theta})=P_s(N_s,N_b)f_s(x_i,\mu,\sigma) + P_b(N_s,N_b) \cdot f_{b}(x_i,\alpha_1,\alpha_2,c)
    \label{fgen}
\end{equation}
where $P_s(N_s,N_b)$ and $P_b(N_s,N_b)$ are respectively the probability for an event of being signal and background. These quantities, which will be equal to the fraction of events of one kind, normalized to the total number of events, can be expressed as 
\begin{equation}
    P_s(N_s,N_b) = \frac{N_s}{N_s+N_b} \ \ \ P_b(N_s,N_b) = \frac{N_b}{N_s+N_b}
\end{equation}
Finally, the likelihood function can be written as 
\begin{equation}
    {\mathcal{L}(\Vec{\theta} \ ) = \prod_{i=0}^{N}{\left(\frac{N_s}{N_s+N_b} \cdot \frac{1}{\sqrt{2\pi\sigma^2}}e^{-\frac{1}{2}\left(\frac{x_i-\mu}{\sigma}\right)^2} + \frac{N_b}{N_s+N_b} \cdot\left( c\cdot \frac{1}{\alpha_1}e^{-\frac{x_i}{\alpha_1}}+(1-c)\cdot \frac{1}{\alpha_2}e^{-\frac{x_i}{\alpha_2}}\right)\right)}}
\label{eq:lik}
\end{equation}

By minimizing \ref{eq:lik} on the data the values of the model parameters which better represent the data are found.

The case of two Gaussian signals can be obtained by modifying equation \ref{fgen} into 
\begin{equation}
    f(x_i,\Vec{\theta})=\sum_{j=1}^{2}P_{sj}(N_{s1},N_{s2},N_b)f_{sj}(x_i,\mu_j,\sigma_j) + P_b(N_s,N_b) \cdot f_{b}(x_i,\alpha_1,\alpha_2,c)
\end{equation}
with $\Vec{\theta}=(N_b,N_{s1},N_{s2},\mu_1,\sigma_1,\mu_2,\sigma_2,\alpha_1,\alpha_2,c)$, and $P_{s1/s2/b}(N_{s1},N_{s2},N_b)=\frac{N_{s1/s2/b}}{N_{s1}+N_{s2}+Nb}$.

\label{sec:analysis}
For the analysis, the modeling, and the fit, the $RooFit$ toolkit has been employed \cite{Verkerke:2003ir}. The minimizer used to find the minimum of $-log(\mathcal{L})$ is MIGRAD from the MINUIT package of RooFit \cite{James:1994vla}.
The results of the fit are shown in figure \ref{fig:fits}, and the parameters are reported in table \ref{tab:fitRes}.

\begin{table}[!ht]
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
    \hline
        Source  & $\alpha_1$ & $\alpha_2$ & $c$ & $\mu_1$ & $\sigma_1$ & $\mu_2$ & $\sigma_2$ \\ \hline
        Ca & -9.5$\times$10$^{-4}$ & -9.71$\times$10$^{-5}$ & 0.24 & 5.064$\times$$10^{3}$ & 1.39$\times$$10^{3}$ & x & x \\ \hline
        Fe & -1.95$\times$10$^{-4}$ & -3.85$\times$10$^{-5}$ & 0.56 & 8.33$\times$$10^3$ & 9.53$\times$10$^2$ & 1.70$\times$10$^4$ & 1.38$\times$10$^3$ \\ \hline
        Rb & -4.19$\times$10$^{-4}$ & -4.98$\times$10$^{-5}$ & 0.22 & 9.81$\times$$10^3$ & 2.49$\times$$10^3$ & 1.508$\times$$10^4$ & 2.33$\times$$10^3$ \\ \hline
        Mo & -6.06$\times$$10^{-4}$ & -4.7$\times$$10^{-5}$ & 0.20 & 9.01$\times$$10^3$ & 2.88$\times$$10^3$ & 1.97$\times$$10^4$ & 2.97$\times$$10^3$ \\ \hline
        Ag & -5.34$\times$10$^{-4}$ & -5.38$\times$10$^5$ & 0.20 & 9.53$\times$10$^3$ & 1.78$\times$10$^3$ & 2.57$\times$10$^4$ & 4.12$\times$10$^3$ \\ \hline
        Ba & -2.45$\times$10$^{-4}$ & -3.82$\times$10$^{-5}$ & 0.36 & 9.83$\times$10$^3$ & 1.40$\times$10$^3$ & 4.15$\times$10$^4$ & 5.28$\times$10$^3$ \\ \hline
        Tb & -2.06$\times$10$^{-4}$ & -3.16$\times$10$^{-5}$ & 0.30 & 8.38$\times$$10^3$ & 1.54$\times$10$^3$ & 6.25$\times$10$^4$ & 8.35$\times$10$^3$ \\ \hline
    \end{tabular}
    \caption{In table the parameters of the fits are reported}
    \label{tab:fitRes}
\end{table}

\begin{figure}
    \centering
    \includegraphics[scale=.14]{figures/CaFit.png}
    \includegraphics[scale=.27]{figures/FeFit.png}
    \includegraphics[scale=.27]{figures/CuFit.png}
    \includegraphics[scale=.27]{figures/RbFit.png}
    \includegraphics[scale=.27]{figures/MoFit.png}
    \includegraphics[scale=.27]{figures/AgFit.png}
    \includegraphics[scale=.27]{figures/BaFit.png}
    \includegraphics[scale=.27]
    {figures/TbFit.png}
    \caption{The results of the fit are shown in order of energy: Ca, Fe, Cu, Rb, Mo, Ag, Ba, and Tb. In the plots, the black dot represents the data in a binned representation, the green curve is the background function, the Gaussian curves are the signal, while the blue line is the sum of $s$ and $b$.}
    \label{fig:fits}
\end{figure}

\subsection{Linearity and energy resolution} 
\label{sec:linereso}
The information on the signal in the fit is contained in the $\mu$ and $\sigma$ parameters of the Gaussian. These indeed represent respectively the mean number of light counts expected as response at a given energy, and the detector resolution at that energy. 
From the fits thus, the response in energy of the detector has been characterized by plotting the mean light response as a function of the energy. Moreover, the energy resolution of the detector has been quantified as the ratio of the Gaussian standard deviation divided by its mean value. The plots of the detector response and energy resolution as a function of the energy are reported in figure \ref{fig:linereso}

\begin{figure}
    \centering
    \includegraphics[scale=.33]{figures/Lin.png}
    \includegraphics[scale=.27]{figures/EReso.png}
    \caption{Left: plot of the detector light response. Right: detector energy resolution as a function of the energy. }
    \label{fig:linereso}
\end{figure}

The analysis shows the detector having a linear response in energy up to 35 keV, while at higher energy a deviation from linearity is observed. The energy resolution obtained is aligned with the typical resolution of a gas detector O(10\%). To model it, the data has been fitted with $Res(E)=\sigma_{E}/E = p_0 + p_1/\sqrt{E}$. The point at 6 keV has been excluded from the fit since the parameter of the reconstruction code has been optimized for that energy. This could potentially bias the fit result. 

The energy resolution data shows a bump in the 12-30 keV range. This observed effect could be attributed to the combination of saturation and the way the electrons release their energy. Indeed as illustrated in figure \ref{fig:multiEtracks}, at energies below 15 keV, the tracks consist mainly of a light spot which increases in light and thus in density with the increasing of the energy. As the density increases, the saturation becomes more important, progressively saturating the light output. Beyond 15 keV, the tracks start to exhibit a tail with a "MIP-like" energy release that does not saturate. As the contribution of the tail starts to be dominant $E>35 keV$ the saturation effect on the tracks becomes negligible restoring the $1/\sqrt{x}$ behavior of the energy resolution.
This observation is supported by the plot shown in figure \ref{fig:LY}. This plot is obtained by dividing the light counts for each energy by the energy itself in keV. Since the light response is directly proportional to the light yield ($LY$) $light \propto LY \cdot E$, this plot shows effectively the light yield of the detector as a function of E.  
\begin{figure}
    \centering
    \includegraphics[scale=.4]{figures/LY.png}
    \caption{The plot shows the detector LY as a function of the track energy. The errors are too small to be appreciated.}
    \label{fig:LY}
\end{figure}
As can be seen by this plot, the LY decreases above 6 keV due to the saturation on light spot tracks. It begins to increase at $\sim$ 20 keV, coinciding with the energy at which the tracks start to show a consistent non-saturated tail. Data at higher energies would be very useful in confirming this behavior.


%\subsection{Signal shape variables unfolding with $_{s}\mathcal{P}\textrtaill{lot}$}
%\label{sec:splot}
%The $_{s}\mathcal{P}\textrtaill{lot}$ technique is used to unfold data distribution. Typically in a dataset, data consists of more than two species (e.g. signal and background). The $_{s}\mathcal{P}\textrtaill{lot}$ technique can be used to statistically separate the contribution of the background from the contribution of the signal. The variables of the data can be divided into two classes. The first class are the discriminating variables, for which the p.d.f. are known. The second class are the control variables, for which the p.d.f. is not known, and the distribution must be determined. The $_{s}\mathcal{P}\textrtaill{lot}$ is a method that estimates the shape of the distribution of the control variables relying on the fit of the discriminating variables. For simplicity, it will be considered the case in which there are two species composing the dataset: signal ($s$) and background ($b$).  
%For the unfolding, a maximum likelihood fit is performed on the discriminating variable. For each event, two "sWeights" are assigned: $_{s}\mathcal{P}_s(y)$ and $_{s}\mathcal{P}_b(y)$. These two quantities represent respectively the "sWeight" for $s$ and $b$ calculated on the discriminating variable $y$. Their values are proportional to the probability of the event being attributed to either signal or background.
%A detailed calculation of this quantity is reported in appendix \ref{app:appendixA}. The distribution of the control variable for signal and background can be determined by constructing the distribution for each class weighting each event respectively by its sWeight $_{s}\mathcal{P}_s(y)$ and $_{s}\mathcal{P}_b(y)$ \cite{Pivk_2005}.
%Since the sWeigths can be positive or negative, the negative sWeigths contribute to the cancellation of the background components from the pure signal distribution, and vice versa.

%From an operative point of view, in each X-ray dataset, the discriminating variable is the light integral. Following the unbinned likelihood fit, the RooStats::SPlot method has been employed to calculate the sWeights for each event in the dataset, which are then used to build the control variables distributions. The control variables selected, which will be then used to compare the topological variables of the simulated tracks with the ones of the data, are length, width, slimness (length/width), density (light/\#pixels), average specific ionization (light/length), mean position of the Gaussian longitudinal profile, standard deviation of the Gaussian longitudinal profile, number of hits and number of pixels of the cluster without zero-suppression.
%The unfolded distributions of these variables from the Ag run are shown in figure \ref{fig:SplotAg}.

%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=.3]{figures/SplotAgRed.png}
%    \caption{In figure the unfolded signal distributions for the quantities chosen for the data-MC comparison are shown.}
%    \label{fig:SplotAg}
%\end{figure}

%As a crosscheck, the distribution of pure background unfolded from the Ag run has been compared with the no-source data, and a good agreement is found. The comparison is shown in figure \ref{fig:SplotAgBkg}.

%\begin{figure}[h]
%    \centering
%    \includegraphics[scale=.3]{figures/SplotAgCosm.png}
%    \caption{In figure the unfolded background distributions for the Ag run are shown and compared with no-source data. The blue cross represents the unfolded background distribution, while the yellow histograms are the no-source data distributions.}
%    \label{fig:SplotAgBkg}
%\end{figure}


==> chapters/neutrino.tex <==
%----------------------------------------------------------------------------------------
%	Background
%----------------------------------------------------------------------------------------
\chapter{Neutrinos}\label{chap:background}

\section{Neutrino in the standard model}
\subsection{Neutrino interactions}
\subsection{Massless neutrino}
\subsection{The oscillation mechanism}


\section{Neutrino beyond the Standard Model}
\subsection{Neutrino masses}
\subsubsection{Seesaw mechanisms}
\subsubsection{Radiative mechanisms}
\subsubsection{Other mechanisms: Leptoquark end extradimensions}
\subsection{Beyond standard model interaction}
\subsubsection{Neutrino magnetic moment}
\subsubsection{Millicharge}
\subsubsection{Altri meccanismi che aumentano la sezione d'urto a bassa energia}




